Hyperparameter Optimization for Unsupervised Outlier Detection

Given an unsupervised outlier detection (OD) algorithm, how can we optimize its hyperparameter(s) (HP) on a new dataset, without any labels? In this work, we address this challenging hyperparameter optimization for unsupervised OD problem, and propose the first systematic approach called HPOD that is based on meta-learning. HPOD capitalizes on the prior performance of a large collection of HPs on existing OD benchmark datasets, and transfers this information to enable HP evaluation on a new dataset without labels. Moreover, HPOD adapts a prominent sampling paradigm to identify promising HPs efficiently. Extensive experiments show that HPOD works with both deep (e.g., Robust AutoEncoder) and shallow (e.g., Local Outlier Factor (LOF) and Isolation Forest (iForest)) OD algorithms on discrete and continuous HP spaces, and outperforms a wide range of baselines with on average 58% and 66% performance improvement over the default HPs of LOF and iForest.

==> abs.tex <==
Given an unsupervised outlier detection (OD) algorithm, how can we optimize its hyperparameter(s) (HP) on a new dataset, without any labels? In this work, we address this challenging hyperparameter optimization for unsupervised OD problem, and propose the first systematic approach called HPOD that is based on meta-learning. HPOD capitalizes on the prior performance of a large collection of HPs on existing OD benchmark datasets, and transfers this information to enable HP evaluation on a new dataset without labels. Moreover, HPOD adapts a prominent sampling paradigm to identify promising HPs efficiently. Extensive experiments show that HPOD works with both deep (e.g., Robust AutoEncoder) and shallow (e.g., Local Outlier Factor (LOF) and Isolation Forest (iForest)) OD algorithms on discrete and continuous HP spaces, and outperforms a wide range of baselines with on average 58% and 66% performance improvement over the default HPs of LOF and iForest.

==> backup_aaai/01intro.tex <==
Although a long list of unsupervised outlier detection (OD) algorithms have been proposed in the last few decades \cite{Aggarwal2013a,Campos2016evaluation,pang2021deep,han2022adbench}, how to optimize their hyperparameter(s) (HP) remains underexplored. Without hyperparameter optimization (HPO) methods, practitioners often use the default HP of an OD algorithm, which is hardly optimal given many OD algorithms are sensitive to HPs. For example, a recent study by Zhao \textit{et al.} reports that by varying the number of nearest neighbors in local outlier factor (LOF) \cite{Breunig2000a} while fixing other conditions, up to 10$\times$ performance difference is observed in some datasets \cite{zhao2021automatic}. The literature also shows that HP sensitivity is exacerbated for deep OD models with more `knobs' (e.g., HPs and architectures) %to optimize 
\cite{ding2022hyperparameter}, which we also observe in this study---deep robust autoencoder (RAE) \cite{zhou2017anomaly} exhibits up to 37$\times$ performance variation under different HPs in several datasets.
% and do not even have default HPs to employ.
% Thus, it is crucial to develop hyperparameter optimization (HPO) methods for unsupervised OD.


% Fig. \ref{fig:lof_hp} illustrates how simple HPs can lead to huge performance variation for a given OD algorithm like LOF \cite{Breunig2000a} (i.e., 140\% in this example), and the default HPs are not optimal and inferior to our proposal. 
% Moreover, many OD algorithms (e.g., robust autoencoder (RAE) by \citet{zhou2017anomaly}) do not have default HPs.
% \textcolor{blue}{show two figures that OD performance varies significantly w.r.t different HPs; also show the default choice is not sufficient.} 

\begin{figure*} [!t]
    \centering
	\subfloat[(left) large perf. variation over 384 HPs for \textbf{RAE} on \texttt{Thyroid}---random\&min. loss HPs are sub-par; (right) \method (\textcolor{dodgerblue}{\textbf{\textit{H}}}) outperforms all.] {%
			\includegraphics[clip,width=0.242\columnwidth]{figs/vplot35_thyroid.pdf}%
		\includegraphics[clip,width=0.46\columnwidth]{figs/RAE_demo_v2.pdf}%
		\label{fig:rae_demo}
	}
	\hspace{0.05in}
	\subfloat[(left) HP sensitivity of \textbf{LOF} on \texttt{Vowels}---the default HP is far from optimal; (right) \method (\textcolor{dodgerblue}{\textbf{\textit{H}}}) outperforms all baselines with +58\% AP rank over random HP.]{%
		\includegraphics[clip,width=0.41\columnwidth]{figs/lof_sensitivity.pdf}%
		\includegraphics[clip,width=0.46\columnwidth]{figs/LOF_demo_v2.pdf}%
	\label{fig:lof_demo}
	}
	\hspace{0.05in}
	\subfloat[Perf. comparison on ensemble \textbf{iForest}; \method (\textcolor{dodgerblue}{\textbf{\textit{H}}}) outperforms all baselines markedly.] {%
		\includegraphics[clip,width=0.46\columnwidth]{figs/iForest_demo_v2.pdf}%
		\label{fig:iforest_demo}
	}
	\vspace{-0.1in}
	\caption{
	(\textit{a}) (left) Demo of HP sensitivity in deep RAE on \texttt{Thyroid}; (right) \method 
% 	is \textit{statistically better} than 
	outperforms
	all baselines on a 39-dataset database (see \S 4.2.1), with a higher avg. performance rank (y-axis) as well as comparable to better top q\% HP settings in the meta-HP set (x-axis) (\textit{b}) (left) HP sensitivity in LOF on \texttt{Vowels}; (right) \method 
	outperforms all baselines with great performance edge (e.g., $+58\%$ normalized AP rank) over the default HP (\S 4.2.2)
% 	is \textit{statistically better} than baselines for LOF except HyperEnsemble (see Table \ref{table:lof_pairs}) 
and (\textit{c}) for iForest, \method is also the best with huge improvement (e.g., $+66\%$ normalized AP rank) over the default HP (\S 4.2.2). See detailed experiment results in \S \ref{sec:exp}.
% datasets details are provided in Appx. Table \ref{appx:datasets}.
% is also \textit{statistically better} than all baselines (see Table \ref{table:iforest_pairs}).
% 	\textcolor{blue}{caption v2} (\textit{i}) HP sensitivity in deep OD models (\ref{fig:rae_demo} left) and classical LOF (\ref{fig:lof_demo} left) and (2) \method are \textit{statistically better} than baselines on a 39-dataset database (see Table \ref{table:rae_pairs}, \ref{?},  \ref{table:iforest_pairs}) for RAE (\ref{fig:rae_demo}), LOF (\ref{fig:lof_demo}), and iForest (\ref{fig:iforest_demo}), with higher avg. performance rank (y-axis) and better comparable performance to top HP settings (x-axis).
	}
	\vspace{-0.25in}
	\label{fig:overall}
\end{figure*}


In supervised learning, one can use % hold-out data with 
ground truth labels to evaluate the performance of an HP, leading to a simple grid and random search \cite{bergstra2012random} and more advanced Sequential Model-based Bayesian Optimization (SMBO) \cite{DBLP:journals/jgo/JonesSW98}. Unlike the simple methods, SMBO builds a cheap regression model (called the surrogate function) of the expensive objective function (which often requires ground truth labels), and uses it to iteratively select the next promising HP for the objective function to evaluate. Notably, learning-based SMBO outperforms simple, non-learnable methods
% without a learning process 
in many applications \cite{thornton2013auto,falkner2018bohb}. 
% than the simple methods.
% \textcolor{blue}{Add a bit more information for BO, mention the surrogate function, and point out that it requires evaluation}.

% Different from supervised setting, 
However, unsupervised OD algorithms face evaluation challenges---they do not have access to (external) ground truth labels, and 
% most non-deep OD algorithms 
most of them 
(e.g., LOF and Isolation Forest (iForest) \cite{liu2008isolation}) do not have an (internal) objective function to guide the learning either.
% neither has it (internal) objective function to guide the learning (for most non-deep OD algorithms including LOF and Isolation Forests (iForest) \cite{liu2008isolation}).
% , do not have an  neither. 
Even for 
% the ones
the OD algorithms 
with an internal objective (e.g., reconstruction loss in RAE), 
% the value of objective function 
its value does not necessarily correlate with the actual detection performance \cite{ding2022hyperparameter}. 
Thus, HPO for unsupervised OD remains underexplored, where the key is reliable model evaluation.
% how to evaluate HP for unsupervised OD remain underexplored, which is the key for HPO.

% existing HPO methods by 
% based on 
% \textit{external} or \textit{internal} evaluation do not
% directly 
% apply to unsupervised OD.
% and HPO methods for unsupervised OD are needed.
% , and using internal objective functions can also be misleading

% hyperparameter tuning for unsupervised OD is vastly unknown and underexplored.
% a ``black-art''.

Moving beyond proposing another detection algorithm, we study this important \underline{H}yper\underline{P}arameter \underline{O}ptimization for unsupervised \underline{OD} %({\prob}) 
problem,
% In this work, we 
and introduce (to our best knowledge) \textit{the first %\prob approach
solution} called \method.
% In a nutshell, \method is an SMBO-style HP tuning method for unsupervised OD algorithms.
In a nutshell, \method leverages meta-learning to enable (originally supervised) SMBO for unsupervised OD hyperparameter optimization.
% under SMBO. 
To overcome 
the infeasibility of evaluation in 
% the aforementioned evaluation challenges in 
% supervised 
unsupervised OD, \method leverages meta-learning that carries over past experience on prior datasets/tasks to more efficient learning on a new task. To that end, we build a meta-database with historical performances of a large collection of HPs on an extensive corpus of existing OD benchmark datasets, 
% . On top of it, 
% we 
and train a \textit{proxy performance evaluator} (\ftrain) 
% (\textcolor{blue}{name to change; this is \methodz}) 
% in place of the true objective function 
to evaluate HPs on a new dataset \textit{without labels}. By plugging 
% this performance evaluator 
\ftrain 
into SMBO, \method can iteratively and efficiently identify promising HPs to evaluate and output the best.
Additionally, we use meta-learning to facilitate SMBO in \method 
by \textit{initializing} and \textit{transferring knowledge} from similar historical tasks to the surrogate function of the new task.
% while benefiting from SMBO's efficient sampling of promising HPs. 
% and improve the selection of promising HPs in SMBO by  
% along with 
% Additionally, we also use meta-learning to  
% to identify more promising HPs with
% \textit{meta-learning-based surrogate function initialization and transfer}.
% \textit{surrogate function initialization} and \textit{knowledge transfer} based on the similarity to historical tasks.
We find it important to remark that \method is strictly an HPO technique other than a new detection algorithm.


\textbf{Performance}. Fig. \ref{fig:rae_demo} (left) shows the huge performance variation (up to 37$\times$) for a set of 384 deep RAE HPs on \texttt{Thyroid} data, where \method is  significantly better than %the HPs by randomly selection 
expectation (i.e. random selection),
as well as selection by min. reconstruction loss (MinLoss); ours is one of the top HPs. %optimality. 
In Fig. \ref{fig:rae_demo} (right), we show that \method is significantly better than a group of diverse and competitive baselines (see Table \ref{table:baseline}) on a 39 dataset database. 
We also demonstrate \method's generality on non-deep OD algorithm LOF with both discrete and continuous HP spaces in Fig. \ref{fig:lof_demo}, as well as the %stable 
popular iForest in Fig. \ref{fig:iforest_demo}. 
% In both cases, 
For all three OD algorithms, 
\method is \textit{statistically} better than (most) baselines, including the default HPs of LOF and iForest which are widely used by practitioners. 
% \la{
In fact, being an ensemble, iForest has been shown to be robust to HPs and outperform many other detectors in the literature \cite{emmott2015meta}. As such, improving over its default setting by our \method is remarkable.
% }
% in \prob.
% illustrates how simple HPs can lead to huge performance variation for a given OD algorithm like LOF \cite{Breunig2000a} (i.e., 140\% in this example), and the default HPs are not optimal and inferior to \method.

% None of them are continuous. Table

In summary, the key contributions of this work include:

	\cbit
	\item \textbf{First 
	HPO framework 
% 	Hyperparameter Optimization 
	for Unsupervised Outlier Detection}. We introduce \method, a novel meta-learning approach 
% 	for \prob. It 
	that 
	capitalizes on historical OD tasks with labels to select effective HPs for a new task without any labels.
	\item \textbf{Continuous HP search}. 
	Superior to 
% 	Better than the 
	 baselines in Table \ref{table:baseline}, \method works with both discrete \textit{and} continuous HPs. 
	\item \textbf{Generality and Effectiveness}. Extensive results on 39-datasets with (\textit{a}) deep method RAE and classical methods (\textit{b}) LOF and (\textit{c}) iForest show that \method is markedly better than 
% 	a wide range of 
	leading baselines,  with on avg. 58\% and 66\% improvement over the default HPs of LOF and iForest.
% 	\item \textbf{Effectiveness}. \textcolor{blue}{bragging about the performance; statistically better than default on iForest and LOF. Refer to some results in Fig \ref{fig:overall}}
% 	\item \textbf{Open-source Platform}. We release\footnote{\url{}} \method and our meta-learning database for the community to use in practice
% 	\textcolor{blue}{remove for more space}
	\ceit
\textbf{Reproducibility}. To foster future work on HPO for OD, we open-source all code and env. at \url{https://tinyurl.com/hpod22}.




==> backup_aaai/02related.tex <==

\input{tables/baseline}
\subsection{Hyperparameter Optimization (HPO) for OD}
% Although there is no shortage of outlier detection algorithms, (to our best knowledge) all 
We can categorize the short list of HPO methods for OD into two.
The first group of methods require a hold-out set with ground truth labels for evaluation \cite{bahri2022automl}, including AutoOD \cite{li2021autood}, TODS \cite{lai2021revisiting}, and PyODDS \cite{li2020pyodds}, which do not apply to unsupervised OD scenarios. The second group of methods uses the default HP in the paper, randomly picking an HP, selecting the HP by internal objective/evaluation  \cite{goix2016evaluate,marques2020internal}, or averaging the outputs of randomly sampled HPs \cite{wenzel2020hyperparameter};
% , where 
we include them as baselines (see col. 2-5 of Table \ref{table:baseline}) 
with empirical results in \S \ref{subsec:exp_results}.

\vspace{-0.075in}
\subsection{Hyperparameter Opt. and Meta-Learning}
\label{subsec:hpo_meta_learning}
\vspace{-0.025in}

HPO gains great attention due to its advantages in searching and optimizing through complex HP spaces, where learning tasks are costly \cite{karmaker2021automl}. Existing methods include simple grid and random search \cite{bergstra2012random} and more advanced Sequential Model-based Bayesian Optimization (SMBO) \cite{DBLP:journals/jgo/JonesSW98}. Notably, SMBO builds a cheap regression model (called the surrogate function) of the expensive objective function, and uses it to iteratively select the next promising HPs to be evaluated by the objective function (see Appx. \ref{appx:SMBO}). 
% it has been widely used in model selection and HP optimization \citep{bergstra2015hyperopt}.
% We want to remark 
% Note that 
We cannot directly use these supervised methods, % in \prob, 
rather, \method leverages meta-learning to enable 
% (supervised) 
SMBO 
for \textit{HPO for OD}.

% Grid and random search. SMBO (\textcolor{red}{Just say it is supervised and the key is to identify promising HPs}). Sequential Model-based Optimization (SMBO) is designed for efficiently optimizing expensive global continuous objective functions by optimizing a cheaper surrogate function \citep{hutter2011sequential};  

Meta-learning aims to facilitate the new task learning by leveraging and transferring knowledge from prior/historical tasks \cite{vanschoren2018meta}, which has been used in warm-starting SMBO \cite{feurer2014using} and transferring surrogate in SMBO \cite{yogatama2014efficient,wistuba2016two,wistuba2018scalable}. Recently, meta-learning has also been applied to unsupervised outlier model selection (UOMS), where Zhao \textit{et al.} proposed MetaOD \cite{zhao2021automatic} with comparison to baselines including global best (GB), ISAC \cite{conf/ecai/KadiogluMST10}, and ARGOSMART (AS) \cite{nikolic2013simple}. We adapt these UOMS methods as baselines for HPO for OD (see col.
6-9 of Table \ref{table:baseline}). Although these  leverage meta-learning, they cannot tackle continuous HPO. \method outperforms them in all experiments (see \S \ref{subsec:exp_results}).   
% , and HP space pruning
% Works on surrogate transfer 

% \subsection{Preliminary on Sequential Model-based Optimization (SMBO)
% % \textcolor{blue}{move to a separate section (e.g., related work and preliminary?)}
% }
% % \textcolor{blue}{Present the basics of SMBO and then point out its infeasibility in \prob. Need a sentence for transition.}
% % Sequential Model-based Optimization (SMBO) 
% SMBO methods are designed for efficiently optimizing expensive global continuous objective functions by optimizing a cheaper surrogate function \citep{hutter2011sequential}; it has been widely used in model selection and HP optimization \citep{bergstra2015hyperopt}. For HPO tasks, SMBO methods construct a regression model (i.e., surrogate function) and use it for identifying the promising HPs to be evaluated by the true objective function. It iterates between fitting the surrogate function with newly evaluated HP information and gathering new information based on the surrogate function. Notably, SMBO introduces a class of HP selection criteria called acquisition functions to pick the HP settings with high performance and potential.

% % , i.e.,  

% Appx. \ref{appx:SMBO} Algorithm \ref{algo:smbo} shows the pseudo code of classical SMBO for HPO. In each epoch, the surrogate function predicts the performance and uncertainty of a large number of sampled HP settings, where the acquisition function selects the best one to be evaluated next by the objective function. With the newly evaluated pair of HP settings and the objective value, the surrogate function is updated to be more accurate iteratively. \textcolor{blue}{Clearly, the classical SMBO does not apply to \prob directly since the objective function cannot be evaluated without ground truth labels (Appx. Algorithm \ref{algo:smbo} line 4).}

==> backup_aaai/03method.tex <==
\subsection{Problem Statement}
We consider the hyperparameter optimization (HPO) problem for unsupervised outlier detection (OD), referred to as %\textcolor{red}
\textit{HPO for OD} hereafter. Given a new dataset $\bD_{\text{test}} = (\bXs, \emptyset)$ \textit{without any labels} and an OD algorithm $M$ with the HP space $\vLambda$, the goal is to identify a HP setting $\vlambda \in \vLambda$ so that model $M_\vlambda$ (i.e., detector $M$ with HP $\vlambda$) achieves the highest performance\footnote{\label{footnote:metric}In this paper, we use the area under the precision-recall curve (AUCPR, a.k.a. Average Precision or AP) as the
% objective function/
performance metric, which can be substituted with any other metric of interest.}. 
% given objective function (or evaluation metric) $\mathcal{L}$(\textcolor{red}{consider to change symbol})
HPs can be discrete and continuous, leading to an infinite number of candidate HP configurations. For instance, given $h$ hyperparameters $\lambda_1 \dots \lambda_h$, with domains $\Lambda_1, \dots, \Lambda_h$, the hyperparameter space $\vLambda$ of $M$ is a subset of the cross product
of these domains: $\vLambda \subset \Lambda_1 \times \dots \times \Lambda_h$. Eq. \eqref{eq:hp_opt} presents the goal formally.
% the formal goal of \prob.

\vspace{-0.1in}
\begin{equation} \label{eq:hp_opt}
% \vlambda^* \in 
\argmax_{\vlambda \in \vLambda} \;\;
% \frac{1}{k} \sum_{i=1}^{k} 
% \mathcal{L}
\text{perf}
(M_\vlambda, \bXs)
\end{equation}

\vspace{-0.1in}
\begin{problem}
% [HPO for Unsupervised OD (\prob)]
[HPO for OD]
\textit{\em Given} a new input dataset (i.e., detection task\footnote{Throughout text, we use \textit{task} and \textit{dataset} interchangeably.}) $\mDs = (\bXs, \emptyset)$  without any labels, 
\textit{\em pick} a hyperparameter setting $\vlambda \in \vLambda$ for a given detection algorithm $M$ to employ on $\bXs$ to maximize its performance.
% the objective function $\mathcal{L}$.
\end{problem}
\vspace{-0.05in}

% \la{Note that not all $\vlambda \in \vLambda$ can be evaluated since $\vLambda$ can be infinitely large in case of continuous HP(s), thus a key challenge is efficiently searching the space.}
It is infeasible to evaluate an infinite number of configurations with continuous HP domain(s), and thus
% $\vlambda \in \vLambda$ with continuous HP(s), 
% where it can be infinitely large with continuous HP(s); 
a key challenge is efficiently searching the space.
Further, since \textit{HPO for OD} does not have access to ground truth labels $\mathbf{y}_{\text{test}}$,
% $\mathcal{L}$ 
HP performance (perf.)
cannot be evaluated directly.
\vspace{-0.1in}


\subsection{Overview of \method}
\label{subsec:overview}

% \subsubsection{Overview} 
% \textcolor{blue}{Given overview/flow of \method, and point to the details below? Given an updated pseudo-code to classical SMBO}

In \method, we use \textit{meta-learning} to enable (originally supervised) SMBO for \textit{HPO for OD}, where the key idea is to transfer useful information from historical tasks to a new test task. As such, \method takes as input a collection of historical tasks 
$\mDt = \{\mD_1,\ldots,\mD_n\}$, namely, a meta-train database with ground-truth labels where $\{\mD_i = (\bX_i,\by_i)\}_{i=1}^n$. Given an OD algorithm $M$ for HPO, we define a finite meta-HP set 
% with $m$ HP settings 
by discretizing continuous HP domains (if any) to get their cross-product, i.e.,  
$\vlambda_{\mathbf{meta}} = \{\vlambda_1, \ldots, \vlambda_m \} \in \vLambda$. We use $M_j$ to denote detector $M$ with the $j$-th HP setting $\vlambda_j \in \vlambda_{\mathbf{meta}}$.
% $\vlambda_{\mathbf{m}} \in \vLambda$. 
% \textcolor{red}{or $\vlambda_{\mathbf{meta}}$?} 
% By pairing $M$ with $\vlambda_{\mathbf{meta}}$, (without confusion) we have a set of models $\mM = \{M_1 , \ldots, M_m\}$.
\method uses $\mDt$ to compute:
\cbit
\item the historical output scores of each detector $M_j$
% with HP setting $\vlambda_j \in \vlambda_{\mathbf{meta}}$ 
on each meta-train dataset $\mD_i \in \mDt$, where $\mO_{i,j} := M_j(\mD_i)$ refers to the output outlier scores using the $j$-th HP setting for the points in the $i$-th meta-train dataset $\mD_i$; 
and 
\item the historical performance matrix $\bP\in \R^{n\times m}$  
of each detector $M_j$,
% with HP setting $\vlambda_j \in \vlambda_{\mathbf{meta}}$,
where $\bP_{i,j}:=\text{perf}(\mO_{i,j})$ is $M_j$'s performance\footnotemark[\ref{footnote:metric}]
on meta-train dataset $\mD_i$. 
\ceit

\method consists of two phases. During \textbf{the (offline) meta-learning}, it leverages meta-train database with labels to build a \textit{proxy performance evaluator} (\ftrain), which can predict HP performance 
% of OD algorithm 
on a new task without labels. Also, it trains a \textit{meta-surrogate function} (\ffree) for each meta-train dataset to facilitate later HPO on a new dataset. In the \textbf{(online) HP Optimization} for a new task, \method uses \ftrain to predict its HPs' performance without using any labels, under the SMBO framework to identify promising HP settings in iteration effectively. Also, we improve the surrogate function in SMBO by transferring knowledge 
% (e.g., \ffree) 
from \textit{similar} meta-train datasets.
% and pre-trained \ffree. 
An outline of \method is given in Algorithm \ref{algo:hpod}, where we elaborate on the details of offline meta-training and online \textit{HPO for OD} in \S \ref{subsec:meta_train} and \S \ref{subsec:online_hpo}, respectively.
% \textcolor{red}{AAAI template does support subsubsection index}

\input{algo_hpod}


\subsection{(Offline) Meta-training} 
\label{subsec:meta_train}

% \textcolor{blue}{Discuss what should be done during meta-train}.


In principle, meta-learning carries over the prior experience of historical (meta-train) tasks to do better on a new task, given the latter at least resembles some of the historical tasks. 
% In the following section, we introduce how to use meta-learning to enable HP evaluation in \prob. 
Due to the lack of ground truth labels and/or a reliable internal objective function,  the key challenge in HPO for OD is to evaluate the performance of HP settings. Thus, the core of \method's meta-learning is \textit{learning} the mapping from \textit{HP settings} onto \textit{ground-truth performance} by the \textit{supervision} from the meta-train database. The first part (lines 1-7) of Algorithm \ref{algo:hpod} describes the core steps, and we further discuss on how to learn this mapping (\S 3.3.1) and transfer additional info. for a new task (\S 3.3.2) in the following.

\vspace{-0.05in}

\subsubsection{3.3.1~Proxy Performance Evaluator (\ftrain).} 
\label{subsec:f_train}
% (\textcolor{blue}{this is f-train; name to change}).
In \method, we learn a regressor \f across all meta-train datasets, named \textit{Proxy Performance Evaluator}, that maps their  
\{\texttt{HP settings}, \texttt{data characteristics}, \texttt{additional signals}\} onto ground truth performance.
% \textcolor{red}{(too complex)}.
% and (\textit{ii}) consider similarity among a new task and meta-train tasks to make an accurate prediction. 
% Without dataset characteristics as part of the input,
If \f only uses HP settings as the input feature,
% (i.e., the 1st input term), 
it fails to capture the performance variation of an HP given different datasets.
% differentiate the performance variation of the same HP across different datasets, and may output the average across all. 
Thus, we need additional input features to enable \f for quantifying dataset similarity, so that \f can make similar HP performance predictions on similar datasets, and vice versa.
% the HP performance prediction of \f on two similar datasets stays close, and vice versa.

% How to characterize a dataset for outlier detection? 
How can we capture dataset similarity in OD? 
Recent work by %Zhao \textit{et al.} 
\citep{zhao2021automatic} introduced specialized OD meta-features (MF)  to describe general characteristics of OD datasets; e.g., number of samples, basic feature statistics, etc. With the meta-feature extractor, both meta-train datasets and (later) the test dataset can be expressed as fixed-length vectors, and thus any similarity measure applies, e.g., Euclidean distance. To build \f, we extract meta-features from each meta-train dataset as
$\bM= \{\mathbf{m}_1, \ldots, \mathbf{m}_n\}=\psi(\{\bX_1, \ldots, \bX_n\})\in \mathbbm{R}^{n \times d}$,
% as shown in Eq. (\ref{eq:meta-features}), 
where $\psi(\cdot)$ is the extraction module, and $d$ is the number of MF.

% \begin{equation}
%     \label{eq:meta-features}
%     % \vspace{-0.05in}
%     \bM= \{\mathbf{m}_1, \ldots, \mathbf{m}_n\}=\psi(\{\bX_1, \ldots, \bX_n\})\in \mathbbm{R}^{n \times d}
%     % \vspace{-0.05in}
% \end{equation}

Although meta-features describe general characteristics of OD datasets, their similarity does not necessarily correlate with the \textit{actual performance}. Thus, we enrich the input features of \f  with internal performance measures (IPMs) \citep{ma2021large}, which are more ``performance-driven''. 
 IPMs are noisy/weak unsupervised signals that are solely based on the input samples and/or a given model's output (e.g., outlier scores)
that can be used to compare two models \cite{goix2016evaluate,marques2020internal}. 
% However, they are noisy/weak indicators of performance \cite{ma2021large}. 
In \method, we make the best use of these weak signals by \textit{learning} in \f to regress the IPMs of a given HP setting (along with other signals) onto its true performance \textit{with supervision}.
To build \f, we extract IPMs of 
each detector $M_j$ with HP setting $\vlambda_j \in \vlambda_{\mathbf{meta}}$ on each meta-train dataset $\mD_i \in \mDt$, where $\bIij := \phi(\mO_{i,j})$ refers to the IPMs using the $j$-th HP setting
% for the points in 
for the $i$-th meta-train dataset, and $\phi(\cdot)$ is the IPM extractor. We defer the details on IPMs to Appx. \ref{appx:ipm}.

Putting these together, 
% we first iterate over each meta-train dataset $\mD_i \in \mDt$ to get meta-features $\bM= \{\mathbf{m}_1, \ldots, \mathbf{m}_n\}$, and then compute IPMs $\bI$ of each HP in meta-HP on each meta-train dataset. 
we build \textit{Proxy Performance Evaluator} \f to
% named \textit{Proxy Performance Evaluator}, 
map 
% each 
\{\texttt{HP setting}, \texttt{meta-features}, \texttt{IPMs}\} of HP $\vlambda_j \in \vlambda_{\mathbf{meta}}$ on the $i$-th meta-train dataset onto its 
% corresponding
ground truth performance, i.e.,
$f(\vlambda_j, \mathbf{m}_i, \bIij) \mapsto \bP_{i,j}$. 
See training details of \f in Appx. \ref{appx:ftrain}.

We find it critical to remark that provided $\psi(\cdot)$, $\phi(\cdot)$, and the trained \f  at test time, predicting the detection performance of HP settings becomes possible for the new task without using any ground-truth labels. 

\subsubsection{3.3.2~Meta-Surrogate Functions (\ffree).} Different from \f  that trains on \textit{all} meta-train datasets and leverages \textit{rich input features} (i.e., HPs, MFs, and IPMs) to predict HP performance, we also train $n$ \textit{independent} regressors with \textit{only HPs as input}, $\bm{\mathcal{T}} = \{t_1, \ldots, t_n\}$. That is, for each meta-train dataset $\mD_i \in \mDt$, we train a regressor $t_i(\cdot)$ that simply maps the $j$-th HP setting $\vlambda_j \in \vlambda_{\mathbf{meta}}$ to its detection performance on the $i$-th meta-train dataset, i.e., $t_i(\vlambda_j) \mapsto \bP_{i,j}$.

Since these independent
% and lightweight 
regressors only use HP settings as input, 
% in the offline meta training, 
they can be readily transferred to the online model selection phase to improve HP performance evaluation on $\bXs$. We defer their specific usage to \S 3.4.2 and \S 3.5.2.
\vspace{-0.1in}

% details in Appx. \ref{appx:ffree}.

% \textcolor{blue}{For presentation clarity reasons, we defer a few implementation details to Appx. \ref{appx:offline}, including how to efficiently calculate IPMs, as well as how to train \ftrain and \ffree and use them at test time.} 

% \subsection{(Online) OD Hyperparameter Optimization}
\subsection{(Online) HPO on a New OD Task}
\label{subsec:online_hpo}

After the meta-training phase, \method is ready to optimize HPs for a new dataset. In short, it outputs the HP with the highest predicted performance by \f, the trained performance evaluator (\S 3.4.1). 
To explore 
% unlock 
better HPs efficiently,
% within time budget, 
\method leverages Sequential Model-based Optimization to iteratively select promising HPs for evaluation (\S 3.4.2). The second part (lines 8-18) of Algorithm \ref{algo:hpod} shows the core steps.

% \noindent \textit{Overview}. 
\subsubsection{3.4.1~Hyperparameter Optimization via Proxy Performance Evaluator.} Given a new dataset $\mDs$, we can sample 
a set of 
% a large number of
HPs (termed as the evaluation set $\vlambda_\text{eval} \in \vLambda$), and use the \textit{proxy performance evaluator} \f from meta-training to predict their performance, based on which we can output the one with the highest predicted value as follows.
% (in Eq. (\ref{eq:selected_hp})).
% , as shown in Eq. (\ref{eq:selected_hp}). 
% \textcolor{blue}{to mention \f  with random sampling is already a baseline}

\vspace{-0.1in}
\begin{equation}
\vspace{-0.05in}
    \argmax_{\vlambda_k \in \vlambda_{\text{eval}}} \; f(\vlambda_k, \bmt, \bItk)
    \label{eq:selected_hp}
    % \vspace{-0.05in}
\end{equation}

By setting $\vlambda_{\text{eval}}$ to some \textit{randomly sampled HPs} and plugging it into Eq. (\ref{eq:selected_hp}), 
% for \f  to evaluate and then outputting the highest,
we have the ``version 0" of \method, referred as \methodz.
% for OD HPO.
However, \f  needs IPMs (i.e., $\bItk$ in Eq. (\ref{eq:selected_hp})) as part of the input, requiring detector building at test time. 
% and extracting IPMs requires detector building at the test time. 
Thus, we should construct $\vlambda_{\text{eval}}$ carefully to ensure it captures promising HPs, where random sampling is insufficient.
% . Of course, random sampling has no such guarantee.
% to provide promising HP candidates.
% , and thus selecting from HP 
% model building for them is inefficient.
% is inefficient in budget. 
% Here is the ask: 
Thus we ask: how can we efficiently identify promising HPs for model building and evaluation at  test time? 
% In most cases, we cannot afford to randomly sample HPs, build OD models for generating IPMs, and then feed into \f. 
\vspace{-0.05in}

\subsubsection{3.4.2~~Identifying Promising HPs 
% to the Evaluation Set 
% Promising HPs 
by Sequential Model-based Optimization (SMBO).}
% \subsubsection{3.4.2. Sampling Promising HPs by Sequential Model-based Optimization (SMBO).}
As we briefly described in \S \ref{sec:related}, SMBO can iteratively optimize an expensive objective \citep{hutter2011sequential}, and has been widely used in supervised model selection and HPO \citep{bergstra2015hyperopt}. Other than sampling HPs randomly, learning-based SMBO shows better efficiency in finding promising HPs to evaluate in iterations. 
In short, 
% For an HPO task, 
SMBO constructs a cheap regression model (called surrogate function \s) and uses it for identifying the promising HPs to be evaluated by the (expensive) true objective function. It then iterates between fitting the surrogate function with newly evaluated HP information and gathering new information based on the surrogate function. We provide the pseudo-code of the \textit{supervised} HPO by SMBO in Appx. Algorithm \ref{algo:smbo}, and note that it does not 
% (supervised) SMBO does not
directly 
apply to \textit{HPO for OD} as perf. cannot be evaluated without ground truth labels (line 4).
% of the pseudo-code).

We enable (originally \textit{supervised}) SMBO for \textit{unsupervised} outlier detection HPO by plugging the \ftrain \f from the meta-train in place of HP performance evaluation. The key steps of online HPO by \method are presented below.

\noindent \textbf{\textit{Surrogate Function and Initialization}}. As an approximation of the expensive objection function, surrogate function \s only takes HP settings as input, aiming for fast performance evaluation on a large collection of sampled HPs.
% in \method is designed for fast evaluation on a large collection of sampled HP settings, via approximating the expensive ground truth objective with only HPs, i.e., learning a mapping from an HP $\vlambda_j$ to its ground truth performance $\mathbf{P}_{\text{test}, j}$. 
For the new task $\bXs$ without 
access to true performance evaluation,
% the labels to get ground truth performance, 
\method lets \s learn a mapping from an HP $\vlambda_k$ to its predicted performance, 
% $\widehat{\mathbf{P}}_{\text{test},k}:= f(\vlambda_k, \mathbf{m}_\text{test}, \bItk)$, 
i.e.,  $s(\vlambda_k) \mapsto f(\vlambda_k, \mathbf{m}_\text{test}, \bItk)$. To enable \f on $\bXs$, \method needs one-time computation for the corresponding meta-features as $\mathbf{m}_{\text{test}}:=\psi(\bXs) \in \mathbbm{R}^{d}$. 
We want to remark that \s differs from \f in two aspects. 
First, \s can make fast performance predictions on HPs as it only needs HPs as input, while \f is more costly since IPMs $\bItk$ require model building.
% \f is more costly than \s as IPMs $\bItk$ require model building, while \s only needs HP settings as input for fast prediction. 
Second, \s is a regression model that can measure both \textit{the predicted performance} of HP settings and \textit{uncertainty (potential) around the prediction} simultaneously.
% , so that we could consider both its performance and potential si
% HP candidates' high predicted performance and uncertainty/potential can be measured simultaneously. 
A popular choice for \s is the Gaussian Process (GP)  \citep{williams1995gaussian}\footnote{\label{footnote:gp}We use GP in \method; one may use any regressor with prediction uncertainty estimation, e.g., random forests \citep{breiman2001random}.}. 

To initialize \s, we train it on a small number of HPs.
% , called the initial set $\vlambda_{\mathbf{init}}$. 
More specifically, we train \s with pairs of HPs and their corresponding predicted performance by \f on $\bXs$, and also initialize the evaluation set $\vlambda_{\text{eval}}$ to these HPs. 
% , i.e., $\langle \vlambda, f\rangle$
Although we can randomly sample the initial HPs,
% set $\vlambda_{\mathbf{init}} \in \vLambda$, 
we propose to set them to top-performing HPs from similar meta-train tasks.
% for initialization. 
Consequently, our initial \s 
% has a better prediction of the 
is more accurate in predicting 
likely well-performing HPs on $\bXs$.
% since the first iteration.
We defer the details of this meta-learning-based
% meta-learning-based 
surrogate initialization to \S 3.5.1.

% Notably, SMBO introduces a class of HP selection criteria called acquisition functions to pick the HP settings with both high performance and potential.

% , i.e.,  


\noindent \textbf{\textit{Iteration: Identifying Promising HPs}.} Although we can already output an HP from $\vlambda_{\mathbf{eval}}$ with the highest predicted performance after initialization,
% after the initialization, 
% the goal is 
we aim to use \s to identify ``better and better'' HPs within the time budget.

Under the SMBO framework, in each iteration we use \s to predict the performance (denoted as $u_k:=s(\vlambda_k)$) and the uncertainty around the prediction (denoted as $\sigma_k$) of 
% randomly 
sampled $\vlambda_k \in \vlambda_{\mathbf{sample}}$\footnote{\label{footnote:sample}
$\vlambda_{\mathbf{sample}}$ is a finite HP candidate set that is randomly sampled from the full (continuous) HP space $\vLambda$ 
(see %sampling 
details in Appx. \ref{appx:sampling}).
Since \s can make fast predictions, $\vlambda_{\mathbf{sample}}$'s size can be large, e.g., 10,000 as in \cite{hutter2011sequential}.
% and its size can be large, e.g., 10,000 in \cite{hutter2011sequential}, as \s can make fast prediction 
% on a large number of HP candidates.
},
% $\footnote{$\vlambda_{\mathbf{sample}} \subset \vLambda$ is a randomly sampled finite candidate set. As \s is fast to run, $|\vlambda_{\mathbf{sample}}|$ can be large, e.g. 10,000 \cite{hutter2011sequential}} 
% \ck{(where $$ )}
% \la{there is issue here: $\vLambda$ is the complete/infinite HP space/domain. In SMBO, you sample a finite number (like footnote: The size of $\vlambda_{\mathbf{sample}}$ can be large, e.g. 10,000 \cite{}, since $s(\cdot)$ is extremely cheap. how many do you sample?) of HPs from this space, and that finite set should have a different notation, like $\vlambda_{\mathbf{sample}} \subset \vLambda$} 
and then select the most \textit{promising} one to be ``evaluated'' by \f. 
% \ck{Note $\vlambda_{\mathbf{sample}} \subset \vLambda$ 
% , i.e., 
% and $\sigma_k$ is $u_k$'s prediction uncertainty. 
% $u_k, \sigma_k :=s(\vlambda_k)$. 
% To select an HP to evaluate based on the 
% high predicted performance 
Intuitively, we would like to evaluate the HPs with both high predicted performance $u_k$ (i.e., exploitation) and 
% in a less explored HP space with 
high potential/prediction uncertainty $\sigma_k$ (i.e., exploration), which is widely known as ``exploitation-exploration trade-off'' \cite{shahriari2015taking}. Too much exploitation (i.e., always evaluating the similar HPs) will fail to identify promising HPs, while too much exploration (i.e., only considering high uncertainty HPs) may lead to low-performance HPs. Also, note that the quality of identified HPs depends on the prediction accuracy of \s, where we propose to transfer knowledge from meta-surrogate functions $\bm{\mathcal{T}}$ by performance similarity (see details in \S 3.5.2.)

How can we effectively balance the trade-off between exploitation and exploration in \method? 
As a SMBO method,
% Under the SMBO framework, 
we use the acquisition function \aq to factor in the trade-off and pick a promising HP setting based on the outputs of the surrogate function. 
The acquisition function 
% It 
quantifies the ``expected utility'' of HPs by balancing their predicted performance and the uncertainty.
% around the prediction. 
Thus, we output the most promising HP
% in iteration $e$ 
to evaluate by maximizing \aq:
% , which is generally known as ``exploitation-exploration trade-off''. 

\vspace{-0.1in}


\begin{equation}
% \vspace{-0.025in}
    \vlambda 
    % \vlambda^{(e)} 
    := \argmax_{
    \vlambda_k \in 
    \vlambda_{\mathbf{sample}}
    %\vLambda
    } \;\;
    a(s(\vlambda_k))
    % a(s^{(e)}(\vlambda_k))
    % a(\vlambda_k|s^{(e)})
        \vspace{-0.025in}
    \label{eq:acqusition}
\end{equation}


One of the most prominent choices of \aq is Expected Improvement (EI) \citep{DBLP:journals/jgo/JonesSW98}, which is used in \method and can be replaced by other choices. EI has a closed-form expression
under the Gaussian assumption, and the EI value of HP setting $\vlambda_k$ is shown below.
% \textcolor{red}{symbol to change once we finalize other parts.}

\vspace{-0.15in}
\begin{equation*}
\label{eq:EI}
%\vspace{-0.05in}
    % EI(\vlambda_k|\bX_{\text{test}}, M, s)
    % EI(\vlambda_k|s)
    EI(s(\vlambda_k))
    :=\sigma_{k} \cdot [u_{k} \cdot
    \Phi(u_{k})+\varphi(u_{k})], \quad \text{where}
    \vspace{-0.05in}
\end{equation*}
\begin{equation}
 u_{k}= 
\begin{cases}
    \frac{u_{k}-\widehat{\mathbf{P}}_\text{test}^{*}}{\sigma_{k}}  & \text{if } \sigma_{k} > 0 
    % \quad 
    \textrm{ and } 
    % \quad
    \bigg\{ 0 
    \quad 
    \text{if } \sigma_{k} = 0
\end{cases}
% \;.
\vspace{-0.03in}
\end{equation}

In the above, $\Phi(\cdot)$ and $\varphi(\cdot)$ respectively denote the cumulative distribution and the probability density functions of a standard Normal distribution, $u_{k}$ and $\sigma_{k}$ are the predicted performance and the uncertainty around the prediction of $\vlambda_k$ by the surrogate function \s, and $\widehat{\mathbf{P}}_\text{test}^{*}$ is the highest predicted performance by \f on $\vlambda_{\text{eval}}$  so far. We compare EI with other selection criteria in \S 4.4.1.

At the $e$-th iteration, we plug the surrogate $s^{(e)}(\cdot)$ into Eq. (\ref{eq:acqusition}), which returns $\vlambda^{(e)}$ to evaluate. 
% With the selected $\vlambda^{(e)}$ by Eq. (\ref{eq:acqusition}) at iteration $e$, 
Next, we train the OD model $M$ with $\vlambda^{(e)}$ to get its outlier scores $\mO_{\text{test}}^{(e)}$ and IPMs $\bm{\mathcal{I}}_{\text{test}}^{(e)}$, and then predict its performance by \f as
\begin{equation}
    \widehat{\mathbf{P}}_{\text{test}}^{(e)} :=f(\vlambda^{(e)}, \bmt, \bm{\mathcal{I}}_{\text{test}}^{(e)})
\end{equation}
Finally, we add  $\vlambda^{(e)}$ to the evaluation set
% $\vlambda_{\text{eval}}$ as 
$\vlambda_{\text{eval}} := \vlambda_{\text{eval}} \cup \vlambda^{(e)}$, and update the surrogate function to $s^{(e+1)}$ with newly evaluated HP information
% $\langle$HP, predicted performance$\rangle$ pair, 
% i.e.,  
$\langle\vlambda^{(e)},\widehat{\mathbf{P}}_{\text{test}}^{(e)}\rangle$.

% Putting things together, \method picks the most promising at iteration $e$ as:
% \begin{equation}
%     \vlambda^{(e)} := \argmax_{\vlambda \in \vLambda} EI(\vlambda|\bX_{\text{test}}, M, s^{(e)}, \bm{\mathcal{T}}^{(e)})
% \end{equation}

To sum up, \method alternates between (\textit{i}) identifying the next promising HP 
% to evaluate
by the surrogate function \s and (\textit{ii}) updating \s based on newly evaluated HP. 

% \subsubsection{Termination Criteria}
% \subsubsection{Time Budget~~}
% \label{subsec:termination}

% \ck{
\noindent \textbf{\textit{Continuous HP search}}.
Recall that an outstanding property of \method compared to 
% prior literature 
the baselines
is its capability for continuous HP search (Table \ref{table:baseline}). 
$\vlambda_{\mathbf{sample}}$\footnotemark[\ref{footnote:sample}] can be \textit{any} subset of the full HP space $\vLambda$ and not restricted to the discrete $\vlambda_{\mathbf{meta}}$. 
% }


\noindent \textbf{\textit{Time Budget}}.
As a SMBO method, \method is an \textit{anytime} algorithm: at any time the user asks for a result, it can always output the HP with the highest predicted performance in the evaluation set $\vlambda_{\text{eval}}$ at the current iteration (Eq. (\ref{eq:selected_hp})). \method uses $E$ to denote the max number of iterations.
\vspace{-0.1in}

\subsection{Details of (Online) HPO}
\label{subsec:online_hpo_details}
% \textcolor{red}{consider to move this section to Appendix \ref{appx:online}}
\subsubsection{3.5.1~Meta-learning-based Surrogate Initialization.} 
Other than initializing on a small set of \textit{randomly sampled} HPs, we design a meta-learning initialization strategy for the surrogate function (see \S 3.4.2), based on the similarity between the test and meta-train datasets. Intuitively, we hope the surrogate function \s can make accurate predictions on the top-performing HPs of the test dataset, while the accuracy of the under-performing HP regions is less important. To this end, we use the meta-features (see \S 3.3.1) to calculate the similarity between the test dataset to each meta-train task $\mD_i \in \mDt$, and initialize \s with the top performing HPs from \textit{the most similar meta-train dataset}; these HPs may yield good performance on the test dataset as well.
See
% performance 
the comparison to random initialization in \S 4.4.2.


\subsubsection{3.5.2~Surrogate Transfer by Performance Similarity.} As introduced in \S \ref{subsec:hpo_meta_learning}, meta-learning can be used to improve the surrogate function \s in SMBO by transferring knowledge from meta-train datasets. In \method, we train $n$ independent \textit{Meta-Surrogate Functions} (see \S 3.3.2) for $n$ meta-train datasets, $\bm{\mathcal{T}} = \{t_1, \ldots, t_n\}$; each with the same regression function as \s (i.e., Gaussian Process). To this end, we identify the most similar meta-train dataset $\mD_i$ in iteration $e$, and use the test surrogate \s and $\mD_i$'s meta-surrogate $t_i$ together to predict the performance of HP $\vlambda_k$,
% and the uncertainty around the prediction, 
i.e., 

\vspace{-0.1in}
\begin{equation}
u_k :=  s^{(e)}(\vlambda_k)+w_i^{(e)}\cdot t_i(\vlambda_k)
% \vspace{-0.025in}
\end{equation}


\noindent
where $w_i^{(e)}$ 
% \la{is this $\in [0,1]$?} 
is the similarity between the test dataset and $\mD_i$ measured in iteration $e$. Of course, we could use meta-features
% discussed in \S 3.3.1 
to measure the dataset similarity, but its value does not change in iterations and 
% this dataset-level similarity 
always finds the same meta-train dataset to transfer 
% surrogate 
(even for different OD algorithms).
% from the surrogate from it.
% , which is not ideal.
% fail to identify truly similar meta-train datasets by performance.

Instead, we 
% instead to 
(re)calculate the \textit{performance similarity} every iteration based on the HPs in $\vlambda_\text{eval}$ between each meta-train task and the test dataset, and \textit{dynamically} transfer the most similar meta-train dataset's meta-surrogate function. 
% Intuitively, 
Specifically, \method computes a rank-based similarity by weighted Kendall tau \cite{shieh1998weighted}) between each meta-train dataset's ground truth performance and the test dataset's predicted performance by \f on $\vlambda_\text{eval}$ (which gets updated in every iteration).
% , which quantifies the similarity between the ordering of the HP performance of  $\vlambda_\text{eval}$.
% High rank similarity denotes  
% consider $\mD_i$ as the most similar meta-dataset, and transfer its $t_i$ to \s. 
% Weight $w_i^{(e)}$ can be calculated as the  
% How to measure 
See the effect of surrogate transfer in \S 4.4.3.
\vspace{-0.14in}


% \textcolor{blue}{Or move to Appx. \ref{appx:surrogate_transfer}?}


% \subsection{Complexity Analysis}

% \textcolor{blue}{Do we need this given it is under SMBO (most SMBO paper does not have complexity analysis)? Or move to in Appx. \ref{appx:complexity}}





==> backup_aaai/04experiments.tex <==
\subsection{Experiment Setting}
\label{subsec:exp_details}
\vspace{-0.05in}

\textbf{OD Algorithms and Testbed}. We show 
% setting and 
the results of HPO on (\textit{a}) deep RAE in \S 4.2.1
and (\textit{b}) LOF and (\textit{c}) iForest in \S 4.2.2. Each OD algorithm is evaluated on a 39-dataset testbed (Appx. \S \ref{appx:datasets}, Table \ref{table:datasets}).
% for the complete list
Details of each algorithm's HP spaces and the meta-HP set is provided in Appx. \ref{appx:od_details}. 
% For consistency, 
All experiments are conducted on an AMD 5900x@3.7GhZ, 64GB RAM workstation with NVIDIA RTX A6000 GPUs.  
% and \ref{appx:datasets}.

\noindent \textbf{Baselines}. Table \ref{table:baseline} summarizes the baselines
% in this study 
with categorization. We include
(\textit{i}) \textbf{\textit{Simple methods}}: \textbf{(1) Default} always employs the same default/popular HP setting (only if specified in the literature) \textbf{(2) Random} choice of HPs and \textbf{(3) MinLoss} outputs the HP with the lowest internal loss (only applicable to the algorithms with an objective/loss function) and (\textit{ii}) \textbf{\textit{Complex methods}}:
% that adapted from unsupervised OD model selection (they output from an HP from the meta-HP set)
% (\textit{ii}) \textbf{\textit{meta-learning based methods that are originally designed for unsupervised OD model selection (they output from a predefined meta-HPs)}}:  
\textbf{(4) HyperEnsemble (HyperEns} or \textbf{HE)} that averages the results of randomly sampled HPs \citep{wenzel2020hyperparameter}
\textbf{(5) Global Best (GB)} selects the best performing HP on meta-train database on average \textbf{(6) ISAC}  ~\cite{conf/ecai/KadiogluMST10} \textbf{(7) ARGOSMART (AS)} ~\cite{nikolic2013simple} and \textbf{(8) MetaOD} ~\cite{zhao2021automatic}.
Additionally, we include \textbf{(9) \methodz}, a variant of \method that  directly uses \f to choose from randomly sampled HPs (see \S 3.4.1).
% \textcolor{blue}{(9) any other things?} 
% Also note for the detection method with an \textbf{internal objective (IO)} function, e.g., reconstruction error of RAE, and we could also tune HPs by it. \textcolor{blue}{Update this later}. 
Note that the unsupervised OD model selection baselines (5)-(8) are not for \textit{HPO for OD}, i.e. they are infeasible with continuous HP spaces. We adapt them for HPO by selecting 
% an HP 
from the discrete meta-HP set in \S \ref{subsec:overview}.
% as we train \ftrain $f(\cdot)$.
More details of the baselines are in Appx. \ref{appx:baselines}.

\noindent \textbf{Evaluation}.  We split the meta-train/test by leave-one-out cross-validation (LOOCV). Each time we use one dataset as the input dataset for HPO, and the remaining datasets as meta-train. 
We run five independent trials and report the average for the baselines with randomness. 
% e.g., \textbf{(2) Random}. We use 
% the area under the precision-recall curve (Average Precision or AP) 
We use Average Precision (AP) as the performance measure, while it can be substituted with any other measure\footnotemark[\ref{footnote:metric}].
% , e.g., the area under the receiver operating characteristic curve (ROC). 
As the raw performance like AP is not comparable across datasets with varying magnitude, we report the normalized AP rank of an HP, ranging from 1 (the best) to 0 (the worst)---thus higher the better. Also, we provide an additional metric called ``top q\%'', denoting that an HP's performance has no statistical difference from the top q\% HP from the meta HP-set, ranging from 0 (the best) to 1 (the worst)---thus lower the better.
To compare two methods, we use the paired Wilcoxon signed rank test across all 39 datasets
% in the testbed 
(significance level $p$$<$$0.05$).
We give the full performance results in Appx. \ref{appx:full_results}.

\noindent \textbf{Hyperparameters}. The hyperparameters of \method are chosen by LOOCV on the meta-train set. To that end, we initialize the surrogate function with 10 HPs. Also, 
we report the results within a 
% cross-validation to decide \textcolor{red}{add then}, and 
30-minute budget for deep RAE and 10-minute budget for LOF and iForest, leading to $E$=40 iters.

% \noindent \textbf{OD algorithms and hyperparameters}. We provide details on the HP space and the meta-HP set of RAE, LOF, and iForest in \ref{appx:od_details}.
\vspace{-0.1in}

\subsection{Experiment Results}
\label{subsec:exp_results}


\subsubsection{4.2.1~Results on (Deep) Robust Autoencoder.}
% \label{subsec:result_rae}
% \begin{figure}[!h]
% %\vspace{-0.1in}
% \centering
% 	\includegraphics[width=\linewidth]{figs/cd-diagram-rae.pdf}
% 	\vspace{-0.25in}
% 	\caption{Comparison of avg. rank (lower is better) of algorithms w.r.t. RAE performance across datasets. \method outperforms all w/ the lowest avg. rank.
% 	Numbers on each line is the avg. AP-rank (lower is better) of the employed HP (selected or otherwise) 
% 	by each method. \textcolor{red}{consider combine as a single figure}
% 	}
% 	\label{fig:cd_plot_rae}
% 	\vspace{-0.1in}
% \end{figure} 
% \input{tables/RAE_pairs}

% As shown in 
Fig. \ref{fig:rae_demo} (right) and \ref{fig:cd_plot_rae} show that \textbf{\method outperforms all baselines w.r.t. both the best avg. normalized AP rank and the top q\% value}. Furthermore, \method is also statistically better than all baselines as shown in Table \ref{table:rae_pairs}, including strong meta-learning baseline MetaOD ($p$$=$$0.0398$). Its advantages can be credited to two reasons. First, meta-learning-based \method leverages prior knowledge on similar historical tasks to predict HP perf. on the new dataset, whereas simple baselines like Random and MinLoss cannot. Second, only \method and \methodz can select HPs from continuous spaces, while other meta-learning baselines 
% can only search through discrete spaces 
% \la{
are limited to finite discrete HPs as specified for the meta-train datasets
% } 
which 
% may be too 
are too few to capture optimal HPs (especially for deep models with huge HP spaces).

% \noindent \textbf{\method and \methodz outperform the meta-learning baselines that are infeasible with continuous HP spaces}. Notably, deep RAE has a huge continuous HP space, which poses challenges for \prob. \method and \methodz (i.e., the top two methods in Fig. \ref{fig:cd_plot_rae}) use  \f to select sampled HPs from continuous spaces, showing 
% % the effectiveness of \f and 
% the benefit of working with continuous HP spaces. In contrast, discrete methods like MetaOD and AD can only output from a limited, discrete meta-HP set with lower performances.
% the meta-learning-based \f. 

\noindent \textbf{HPO by the internal objective(s) is insufficient}. 
% The results show that 
Fig. \ref{fig:cd_plot_rae} shows that selecting HP by minimal reconstruction loss (i.e., MinLoss) has the worst performance for RAE, even if it can work with continuous spaces. This suggests that internal loss does not necessarily correlate with external performance. On avg., \method has 37\% higher normalized AP rank, showing the benefit of transferring supervision via meta-learning.

\begin{figure}[!ht]
    \centering
    \vspace{-0.1in}
    \subfloat[Results on RAE]
    {
    \includegraphics[clip,width=0.8\columnwidth]{figs/cd-diagram-rae-cropped.pdf}
    \label{fig:cd_plot_rae}
    }
    
    % \vspace{-0.05in}
    \subfloat[Results on LOF]
    {
    \includegraphics[clip,width=0.8\columnwidth]{figs/cd-diagram-lof-cropped.pdf}
    \label{fig:cd_plot_lof}
    }
    
    % \vspace{-0.05in}
    \subfloat[Results on iForest]
    {
    \includegraphics[clip,width=0.8\columnwidth]{figs/cd-diagram-iforest-cropped.pdf}
    \label{fig:cd_plot_iforest}
    }
    \vspace{-0.1in}
    \caption{Comparison of avg. rank (lower is better) of algorithm performance across datasets on three OD algorithms. \method outperforms all w/ the lowest avg. algo. rank.
	The numbers on each line are the top q\% value (lower is better) of the employed HP (or the avg.)
% 	(selected or otherwise) 
	by each method. \method shows the best performance in all three HPO experiments.}
    \label{fig:cd_plots}
    \vspace{-0.2in}
\end{figure}
\input{tables/pairs}

\input{tables/case_study}
\subsubsection{4.2.2~~Results on LOF
% with Mixed HP Spaces 
and 
% (Ensemble-based) 
iForest.
% (\textcolor{blue}{short one})
}
% \label{subsec:result_lof}

\noindent In addition to deep RAE, \textbf{\method shows generality on diverse OD algorithms}, including non-deep LOF (Fig. \ref{fig:lof_demo} and \ref{fig:cd_plot_lof}) with mixed HP spaces (see details in Appx. Table \ref{table:rae_lof})
% (i.e., continuous number of neighbors and categorical distance metrics)
as well as ensemble-based iForest (Fig. \ref{fig:iforest_demo} and \ref{fig:cd_plot_iforest}). \method achieves the best performance in both with the best norm. AP rank and top q\%. 

\noindent \textbf{\method is statistically better than the default HPs of LOF ($p$$=$$0.0029$) and iForest ($p$$=$$0.0013$)} (see Table \ref{table:lof_pairs} and \ref{table:iforest_pairs}). More specifically, we find that \method provides $+58\%$ and $+66\%$ performance (i.e., normalized AP rank) improvement over using the default HPs of LOF (Fig. \ref{fig:lof_demo} (right)) and iForest (Fig. \ref{fig:iforest_demo}). In fact, note that the default HPs rank the lowest for both LOF (Fig. \ref{fig:cd_plot_lof}) and iForest (Fig. \ref{fig:cd_plot_iforest}), justifying the importance of HPO methods in unsupervised OD.

\noindent \textbf{HyperEns that averages outlier scores from randomly samples HPs yield reasonable performance}, which agrees with the observations in the literature \cite{ding2022hyperparameter}. However, HyperEns has a higher inference cost as it needs to save and use all base models,
% for prediction, 
not ideal for time-critical applications. Using a single model with the selected HPs by \method offers not only better detection accuracy but also efficiency.
\vspace{-0.1in}


% \noindent \textbf{The benefit of learning-based HPO}. \method is better than \methodz. LOF, iForest, and ablation 

% \subsubsection{4.2.3. Results on (Ensemble-based) Isolation iForest}
% \label{subsec:result_iforest}

% \begin{figure}[!h]
% %\vspace{-0.1in}
% \centering
% 	\includegraphics[width=\linewidth]{figs/cd-diagram-iforest.pdf}
% 	\vspace{-0.25in}
% 	\caption{Comparison of avg. rank (lower is better) of algorithms w.r.t. iForest performance across datasets. \method outperforms all w/ the lowest avg. rank.
% 	Numbers on each line is the avg. AP-rank (lower is better) of the employed HP (selected or otherwise) 
% 	by each method. 
% 	}
% 	\label{fig:cd_plot_iforest}
% 	\vspace{-0.1in}
% \end{figure} 

% \input{tables/iforest_pairs}



\subsection{Case Study}
\label{subsec:case_study}
\vspace{-0.05in}

It is interesting to trace how \method identifies better HPs over iterations given a dataset. We show an example of tuning LOF on \texttt{Cardiotocography} dataset in Table \ref{table:case_study}. Among 200 candidate HP settings 
% \la{remove: in the meta-HP set -- as it suggests you are limited to it and not doing continuous search. not sure what you actually did. no inner grid?}
(see Appx. Table \ref{table:rae_lof}), the optimal HP setting is \{`Chebyshev', 79\} with AP=0.3609. In 30 iterations, \method gradually identifies better HPs (closer to optimal), i.e., \{`Chebyshev', 73\}. Its AP improves from 0.2866 (1-\textit{st} iteration) to 0.357 (30-\textit{th} iteration). See full trace in Appx. \ref{appx:case_study}, Table \ref{table:case_study_full}. 


\subsection{Ablation Studies and Other Analysis}
% \subsection{Additional Analysis}

\subsubsection{4.4.1~The Choices of Acquisition Function.}
\method uses the EI acquisition to select an HP based on the surrogate function's prediction (see \S 3.4.2). We compare it with random and greedy acquisition (latter picks the HP with the highest predicted performance, %without considering its 
ignoring uncertainty) in Fig. \ref{fig:ablation_ei}, where EI-based acquisition shows the best performance.
\begin{figure}[H]
\vspace{-0.1in}
\centering
	\includegraphics[width=0.74\linewidth]{figs/ablation_sampling.pdf}
	\vspace{-0.1in}
	\caption{Ablation of our EI (med.=0.893) vs. the greedy  (med.=0.870) and random acquisition (med.=0.851).
% 	; the former outperforms
	}
	\label{fig:ablation_ei}
	\vspace{-0.1in}
\end{figure} 

\subsubsection{4.4.2~Surrogate Initialization.}
\method uses meta-learning to initialize the surrogate (see \S 3.5.1). Fig. \ref{fig:ablation_init} shows its advantage over random init. with higher performance.

\begin{figure}[H]
\vspace{-0.1in}
\centering
	\includegraphics[width=0.85\linewidth,left]{figs/ablation_init.pdf}
	\vspace{-0.2in}
	\caption{Ablation of meta-initialization (med.=0.893) vs. random initialization (med. =0.874) of surrogate function.
% 	; the former outperforms
	}
	\label{fig:ablation_init}
	\vspace{-0.05in}
\end{figure} 

\subsubsection{4.4.3~The Effect of Surrogate Transfer.} To improve the prediction performance of the surrogate function, \method transfers meta-surrogate functions from 
% the most 
similar meta-train tasks (see \S 3.5.2). 
Fig. \ref{fig:ablation_transfer} shows that this transfer helps find better HPs, demonstrating the added value of meta-learning besides PPE training of \f and surrogate initialization. % with higher median and 3-$rd$ and 4-$th$ quartile.
% No transfer vs. transfer by meta-features vs. transfer by WK
\begin{figure}[H]
\vspace{-0.1in}
\centering
	\includegraphics[width=0.85\linewidth,left]{figs/ablation_transfer.pdf}
	\vspace{-0.15in}
	\caption{Ablation of our w/ surrogate transfer (med.=0.893) vs. without surrogate transfer (med. =0.872).
% 	; the former outperforms
	}
	\label{fig:ablation_transfer}
	\vspace{-0.1in}
\end{figure} 



==> backup_aaai/05conclusion.tex <==
We introduce (to our knowledge) the {\em first systematic hyperparameter  optimization (HPO) approach for unsupervised outlier detection (OD)}. The proposed \method is a meta-learner, and builds on an extensive pool of historical OD benchmark datasets based on which it trains a performance predictor (offline). 
Given a new task without labels (online), %\method identifies promising HPs by a performance predictor trained via meta-learning on the historical tasks. 
it capitalizes on the performance predictor %\method enables 
to enable (originally supervised) sequential model-based optimization for identifying promising HPs iteratively.
Notably, \method stands out from all prior work on \textit{HPO for OD} in being
capable of handling both discrete \textit{and} continuous HP search.
% by (originally supervised) sequential model-based optimization, which is enabled by meta-learning to unsupervised OD with an HP performance predictor. 
Extensive experiments on three (including both deep and shallow) OD algorithms show its generality, where it significantly outperforms a diverse set of baselines. %its performance edge over diverse baselines illustrates its effectiveness. 
Future work will consider joint 
% automatically 
algorithm selection and continuous hyperparameter optimization for unsupervised OD.

==> backup_aaai/abs.tex <==
Given an unsupervised outlier detection (OD) algorithm, how can we optimize its hyperparameter(s) (HP) on a new dataset, without any labels? In this work, we address this challenging hyperparameter optimization for unsupervised OD problem, and propose the first systematic approach called HPOD that is based on meta-learning. HPOD capitalizes on the prior performance of a large collection of HPs on existing OD benchmark datasets, and transfers this information to enable HP evaluation on a new dataset without labels. Moreover, HPOD adapts (originally supervised) sequential model-based optimization to identify promising HPs efficiently. Extensive experiments show that HPOD works with both deep (e.g., Robust AutoEncoder) and shallow (e.g., Local Outlier Factor (LOF) and Isolation Forest (iForest)) OD algorithms on both discrete and continuous HP spaces, and outperforms a wide range of baselines with on average 58% and 66% performance improvement over the default HPs of LOF and iForest.

==> backup_aaai/algo_hpod.tex <==
\begin{algorithm}[!t]
	\caption{\method: Offline and Online Phases}
	\label{algo:hpod}
	\small{
	\begin{algorithmic}[1]
		\REQUIRE (Offline) meta-train database $\mDt = \{(\bX_i, \by_i)\}_{i=1}^n$, OD algorithm $M$, 
% 		model set $\mM = \{M_1 , \ldots, M_m\}$ by pairing the given OD algorithm $M$ with 
% 		$m$ 
		meta-HP set $\vlambda_{\mathbf{meta}} = \{\vlambda_1, \ldots, \vlambda_m \} \in \vLambda$, 
% 		objective function/evaluation metric $\mathcal{L}$; 
		performance evaluation $\text{perf}(\cdot)$;
		(Online) new OD dataset $\mDs=(\bXs, \emptyset)$ (no labels), 
% 		the evaluation set $\vlambda_{\text{eval}}=\{\emptyset\}$, 
		number of iterations $E$
% 		(\textcolor{blue}{consider whether to mention the surrogate})
		\ENSURE (Offline) \method meta-learners; (Online) the selected hyperparameter setting $\vlambda^{*}$ for $\mDs$
		\algrule
		\textcolor{dodgerblue}{$\blacktriangleright$ (Offline) \textbf{Meta-train}: 
		\textit{Learn functions for HP performance prediction}
% 		\textit{Learn a proxy perf. evaluator}
		}
		{{\textcolor{dodgerblue}{\ttfamily{\bf (\S \ref{subsec:meta_train})}}}} 
		\STATE Train detector $M$ with
		HP 
% 		each HP 
% 		setting 
		$\vlambda_j \in \vlambda_{\mathbf{meta}}$ on 
% 		Train each $M_j \in \mM$ on 
		each $\bX_i$ of $\mD_i \in \mDt$ to get outlier scores $\mO_{i,j}$,  $\forall\; i=1\ldots n, \; j=1\ldots m$
		\STATE Evaluate each $\mO_{i,j}$ against ground-truth labels $\by_i$ to get performance matrix $\bP \in \R^{n\times m}$, where 
% 		$\bP_{i,j} := \mathcal{L}(\mO_{i,j} | \by_i)$
		$\bP_{i,j} := \text{perf}(\mO_{i,j} | \by_i)$
		\STATE Extract meta-features (MF) per task, $\bmi := \psi(\bX_i)$ 
% 		\COMMENT{Eq. (\ref{eq:meta-features})}
		\STATE Compute internal perf. measures (IPM), $\bIij := \phi(\mO_{i,j})$ 
		\STATE Train \textit{proxy performance evaluator} (\ftrain) $f(\cdot)$ to predict the performance $\bP_{i,j}$ from the respective \{HP setting
		$\vlambda_j$, meta-features $\bmi$, IPMs $\bIij$\} 
		\mycommenta{\S 3.3.1}
		\STATE Train each \textit{meta-surrogate function} (\ffree) $t(\cdot)$ per meta-train dataset $ \bm{\mathcal{T}} = \{t_1, \ldots, t_n\}$ to predict the perf. $\bP_{i,j}$ from only the respective \{HP setting $\vlambda_j$\} \mycommentb{\S 3.3.2}
		\STATE \textbf{Save} MF extractor $\psi$,  IPM extractor $\phi$, \ftrain $f$, and \ffree $\bm{\mathcal{T}}$
		\algrule
		\textcolor{dodgerblue}{$\blacktriangleright$ (Online) \textbf{HPO on a new task}: \textit{Iteratively identify promising HP settings and output the best one}} {{\textcolor{dodgerblue}{\ttfamily{\bf (\S \ref{subsec:online_hpo})}}}}
		\STATE Extract meta-features of the test dataset $\bmt := \psi(\bXs)$ 
% 		\COMMENT{Eq. (\ref{eq:meta-features})}
		\STATE Initialize surrogate function $s^{(1)}$ and the evaluation set $\vlambda_{\text{eval}}$ by the meta-train database and \ftrain \COMMENT{\S 3.4.1}
% 		; it can predict the test data performance $\mu$ and uncertainty $\sigma$ of HP setting $\vlambda$ on $M$, $\mu, \sigma := s(\vlambda)$ \textcolor{blue}{(to shorten; do not mention $\mu$ and $\sigma$)}
		\FOR[\S 3.4.2]{$e=1$ to $E$} 
% 		\STATE Acquire similar meta-train task(s) by performance similarity and their pre-trained \ffree $\bm{\mathcal{T}}^{(e)}$ \COMMENT{Eq. (\ref{?})}
		\STATE Transfer meta-surrogate functions $\bm{\mathcal{T}}$ to surrogate $s^{(e)}$ by performance similarity to meta-train tasks
		\COMMENT{\S 3.5.2}
		\STATE Get the next promising HP 
		to evaluate by 
		EI on surrogates' prediction, 
% 		by $ s^{(e)}$ and the transferred $\bm{\mathcal{T}}^{(e)})$
		$\vlambda^{(e)} := \argmax_{\vlambda_{k} \in \vlambda_{\mathbf{sample}}} EI(\vlambda_{k}|s^{(e)})$
% 		$\vlambda^{(e)} := \argmax_{\vlambda_{k} \in \vLambda} EI(\vlambda_{k}|\bX_{\text{test}}, M, s^{(e)}, \bm{\mathcal{T}}^{(e)})$
		\STATE Build $M$ w/ $\vlambda^{(e)}$, and get outlier scores $\mO_{\text{test}}^{(e)}$ and IPMs $\bm{\mathcal{I}}_{\text{test}}^{(e)}$
	   %  $	:= \phi(\mO_{\text{test}}^{(e)})$ 
% 		of $M_{\vlambda^{(e)}}$
        
		\STATE Predict perf. of 
% 		$M_{\vlambda^{(e)}}$'s 
		$\vlambda^{(e)}$ 
		 by \f,
		$\widehat{\mathbf{P}}_{\text{test}}^{(e)} :=f(\vlambda^{(e)}, \bmt, \bm{\mathcal{I}}_{\text{test}}^{(e)})$
% 		\STATE $\mathcal{L}^{(e)} := \text{evaluate} \; \mathcal{L}(M_{\vlambda^{(e)}}, \bXs)$
		\STATE Add $\vlambda^{(e)}$ to the evaluation set $\vlambda_{\text{eval}} := \vlambda_{\text{eval}} \cup \vlambda^{(e)}$ 
		\STATE Update to $s^{(e+1)}$ with new pairs of information $\langle\vlambda^{(e)},\widehat{\mathbf{P}}_{\text{test}}^{(e)}\rangle$
		\ENDFOR
		\STATE \textbf{Output} $\vlambda^{*} \in \vlambda_{\text{eval}}$ with the highest predicted perf. \COMMENT{Eq. (\ref{eq:selected_hp})}
% 		evaluated objective function values.
	\end{algorithmic}
	}
% \vspace{-0.05in}
\end{algorithm}
 \setlength{\textfloatsep}{0.1in}


==> backup_aaai/algo_smbo.tex <==
\begin{algorithm}[!ht]
	\caption{SMBO for Supervised Hyperparameter Optimization 
% 	\textcolor{red}{Let us move this to Appendix to save space.}
	}
	\label{algo:smbo}
	\small{
	\begin{algorithmic}[1]
		\REQUIRE learning algorithm $M$, surrogate function \s, input task $\bD_{\text{test}}=\{\bXs, \mathbf{y}_{\text{test}}\}$,
% 		that can be evaluated by 
		objective function $\mathcal{L}(\cdot)$, number of iterations $E$
% 		(which is infeasible in \prob)
		\ENSURE selected hyperparameter setting $\vlambda^{*}$ for $\bD_{\text{test}}$
		\algrule
		\STATE Initialize surrogate function $s^{(1)}$
		\FOR{$e=1$ to $E$}
		\STATE $\vlambda^{(e)} := \argmax_{\vlambda \in \vLambda} EI(\bX_{\text{test}}), \vlambda|M,  s^{(e)}$
		\STATE $\mathcal{L}^{(e)} := \text{evaluate} \; \mathcal{L}(M_{\vlambda^{(e)}}, \bXs, \mathbf{y}_{\text{test}})$ \COMMENT{infeasible for \textit{HPO for OD}}
		\STATE Update to $s^{(e+1)}$ with new information $\langle\vlambda^{(e)},\mathcal{L}^{(e)}\rangle$
		\ENDFOR
		\STATE \textbf{Output} $\vlambda^{*} \in \vlambda^{(1)}, \dots, \vlambda^{(e)}$ with the highest evaluated objective function values
	\end{algorithmic}
	}
\end{algorithm}
% \setlength{\textfloatsep}{0.0in}
% \vspace{-0.1in}

==> backup_aaai/dfn.tex <==
% \newcommand{\method}{{\sc SMBOD}\xspace}
\newcommand{\method}{{\sc HPOD}\xspace}
\newcommand{\methodz}{{\sc HPOD\_0}\xspace}
% \newcommand{\prob}{{HPUOD}\xspace}
\newcommand{\ftrain}{{PPE}\xspace}
\newcommand{\ffree}{{MSF}\xspace}

\newcommand{\f}{{$f(\cdot)$}\xspace}
\newcommand{\s}{{$s(\cdot)$}\xspace}
\newcommand{\aq}{{$a(\cdot)$}\xspace}

\newcommand{\la}[1]{{\color{magenta} LA: #1}}
\newcommand{\ck}[1]{{\color{brown}#1}}

\newcommand{\vTheta}{{\bm{\Theta}}} %
\newcommand{\vtheta}{{\bm{\theta}}}
\newcommand{\vlambda}{{\bm{\lambda}}}
\newcommand{\vLambda}{{\bm{\Lambda}}}

\newcommand{\argmax}{\operatornamewithlimits{argmax}}

\newcommand{\cbit}{\begin{compactitem}}
	\newcommand{\ceit}{\end{compactitem}}
\newcommand{\cben}{\begin{compactenum}}
	\newcommand{\ceen}{\end{compactenum}}
	
\newtheorem{problem}{Problem}
\newtheorem{definition}{Definition}
\newtheorem{property}{Property}
\newtheorem{theorem}{Theorem}
\newtheorem{proof}{Proof}

\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\mM}{\bm{\mathcal{M}}}

\newcommand{\bXs}{\mathbf{X}_{\text{test}}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\by}{\mathbf{y}}

\newcommand{\bP}{\mathbf{P}}
\newcommand{\hP}{\widehat{\mathbf{P}}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bI}{\mathbf{I}}

\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bC}{\mathbf{C}}

\newcommand{\mDt}{\bm{\mathcal{D}}_{\text{train}}}
\newcommand{\mDs}{\bm{\mathcal{D}}_{\text{test}}}
\newcommand{\mD}{\mathcal{D}}

% \newcommand{\mDt}{\mathbcal{D}_{\text{train}}}
\newcommand{\mXs}{\mathbcal{X}_{\text{test}}}
% \newcommand{\mM}{\mathbcal{M}}


\newcommand{\mN}{\mathcal{N}}
\newcommand{\mI}{\mathcal{I}}


\newcommand{\bmij}{\mathbf{m}_{i,j}}
\newcommand{\bmi}{\mathbf{m}_{i}}
\newcommand{\bmt}{\mathbf{m}_{\text{test}}}

\newcommand{\bmijp}{\mathbf{m}_{i,j'}}

\newcommand{\bIij}{\mathbf{I}_{i,j}}

\newcommand{\bItk}{\mathbf{I}_{\text{test},k}}

\newcommand{\bO}{\mathbf{O}}

\newcommand{\mO}{\mathcal{O}}



\newcommand{\algrule}[1][.5pt]{\par\vskip.5\baselineskip\hrule height #1\par\vskip.5\baselineskip}
\makeatother

\newcommand{\LINEFOR}[2]{%
    \STATE\algorithmicfor\ {#1}\ \algorithmicdo\ {#2} \algorithmicend\ \algorithmicfor%
}



% \SetKwRepeat{Do}{do}{while}%
% \SetKwFor{While}{while}{}{end while}%

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\renewcommand{\algorithmiccomment}[1]{\hfill$\blacktriangleright$ #1}
\newcommand{\cdash}{\multicolumn{1}{c}{--} }
\newcommand{\mycommenta}[1]{\hspace{1.4in}$\blacktriangleright$ #1}
\newcommand{\mycommentb}[1]{\hspace{1.05in}$\blacktriangleright$ #1}

==> backup_aaai/tables/RAE_pairs.tex <==
\begin{table}[h]
% \scriptsize
\caption{
Pairwise statistical test results between \method and baselines by Wilcoxon signed rank test. Statistically better method shown in \textbf{bold} (both marked \textbf{bold} if no significance). For HPO on RAE, \method is statistically better than all. }\label{table:rae_pairs}
 \vspace{-0.1in}
\scalebox{0.87}{
\begin{tabular}{lll|lll}
\toprule
\textbf{Ours} & \textbf{baseline} & \textbf{p-value} & \textbf{Ours} & \textbf{baseline} & \textbf{p-value} \\
\midrule
\textbf{HPOD} & AS                & 0.0309           & \textbf{HPOD} & ISAC              & 0.0028           \\
\textbf{HPOD} & Random            & 0.0014           & \textbf{HPOD} & MetaOD            & 0.0398           \\
\textbf{HPOD} & HyperEns          & 0.0382           & \textbf{HPOD} & MinLoss           & 0.0003           \\
\textbf{HPOD} & GB                & 0.0002           & \textbf{HPOD} & HPOD\_0            & 0.0201    \\
\bottomrule
\end{tabular}}
% \vspace{0.05in}
\end{table}

==> backup_aaai/tables/all_iforest_results.tex <==
\begin{table*}[!ht]
    \footnotesize

    \scalebox{0.95}{
    \begin{tabular}{l|lllllll|ll}
    \toprule
    \textbf{datasets}   & \textbf{Random} & \textbf{GB}         & \textbf{ISAC}       & \textbf{AS}         & \textbf{HyperEns}   & \textbf{MetaOD}     & \textbf{Default}    & \textbf{HPOD\_0}    & \textbf{HPOD}       \\
    \midrule
    1\_ALOI             & 0.3979 (3)      & 0.0191 (8)          & 0.5208 (2)          & 0.0868 (7)          & 0.2789 (5)          & 0.1319 (6)          & 0.0035 (9)          & 0.359 (4)           & \textbf{0.7326 (1)} \\
    2\_Annthyroid       & 0.654 (6)       & \textbf{0.9583 (1)} & 0.0764 (9)          & 0.7535 (5)          & 0.5405 (7)          & 0.9236 (3)          & 0.8789 (4)          & 0.5167 (8)          & \textbf{0.9358 (2)} \\
    3\_Arrhythmia       & 0.4879 (6)      & \textbf{0.8924 (1)} & 0.4427 (7)          & \textbf{0.7517 (4)} & 0.8166 (2)          & 0.2188 (8)          & 0.1107 (9)          & 0.6146 (5)          & 0.8125 (3)          \\
    4\_Cardiotocography & 0.481 (6)       & 0.691 (2)           & \textbf{0.9115 (1)} & 0.6319 (3)          & 0.5765 (4)          & 0.4583 (7)          & 0.5433 (5)          & 0.4115 (9)          & \textbf{0.4444 (8)} \\
    5\_Glass            & 0.6021 (3)      & 0.2517 (8)          & 0.4253 (6)          & 0.3993 (7)          & \textbf{0.5606 (4)} & 0.1684 (9)          & \textbf{0.9585 (1)} & 0.5396 (5)          & 0.7795 (2)          \\
    6\_HeartDisease     & 0.526 (8)       & 0.8681 (3)          & 0.9028 (2)          & 0.6997 (5)          & \textbf{0.6042 (7)} & 0.6319 (6)          & 0.09 (9)            & 0.8326 (4)          & \textbf{0.941 (1)}  \\
    7\_InternetAds      & 0.4498 (7)      & 0.8438 (3)          & 0.2465 (8)          & 0.0174 (9)          & \textbf{0.872 (2)}  & \textbf{0.9132 (1)} & 0.4602 (6)          & 0.6438 (5)          & 0.7543 (4)          \\
    8\_PageBlocks       & 0.3183 (7)      & 0.0972 (8)          & 0.6649 (2)          & \textbf{0.3333 (6)} & 0.5066 (5)          & 0.5903 (4)          & 0.0138 (9)          & 0.6167 (3)          & \textbf{0.9688 (1)} \\
    9\_PenDigits        & 0.481 (4)       & 0.026 (9)           & 0.2951 (6)          & \textbf{0.9878 (1)} & \textbf{0.4976 (3)} & 0.8924 (2)          & 0.0623 (8)          & 0.3108 (5)          & 0.1806 (7)          \\
    10\_Pima            & 0.3599 (7)      & 0.0677 (9)          & 0.9583 (2)          & 0.5417 (6)          & 0.6083 (5)          & 0.783 (3)           & 0.1211 (8)          & 0.6215 (4)          & \textbf{0.9861 (1)} \\
    11\_Shuttle         & 0.4844 (5)      & 0.092 (9)           & 0.5035 (4)          & 0.3472 (6)          & \textbf{0.5654 (3)} & 0.309 (7)           & 0.1886 (8)          & \textbf{0.7326 (1)} & 0.6817 (2)          \\
    12\_SpamBase        & 0.5433 (6)      & 0.8958 (4)          & 0.9028 (3)          & \textbf{0.9479 (2)} & 0.5772 (5)          & 0.1823 (9)          & \textbf{1 (1)}      & 0.2563 (7)          & 0.218 (8)           \\
    13\_Stamps          & 0.6298 (5)      & 0.8941 (2)          & 0.434 (8)           & 0.7795 (4)          & 0.6007 (6)          & \textbf{0.1406 (9)} & 0.564 (7)           & 0.8868 (3)          & \textbf{0.9913 (1)} \\
    14\_Waveform        & 0.4844 (6)      & 0.0799 (8)          & \textbf{0.9757 (1)} & 0.3212 (7)          & 0.546 (5)           & 0.6528 (4)          & 0.0138 (9)          & \textbf{0.8441 (3)} & 0.872 (2)           \\
    15\_WBC             & 0.3737 (7)      & 0.1372 (9)          & \textbf{0.7569 (4)} & 0.7917 (2)          & 0.5273 (6)          & \textbf{0.9653 (1)} & 0.1592 (8)          & 0.7563 (5)          & 0.7917 (2)          \\
    16\_WDBC            & 0.526 (8)       & 0.7188 (4)          & 0.6354 (7)          & 0.6389 (6)          & 0.5038 (9)          & 0.8368 (2)          & 0.6903 (5)          & 0.7955 (3)          & \textbf{0.901 (1)}  \\
    17\_Wilt            & 0.5467 (4)      & 0.2882 (8)          & \textbf{0.3264 (6)} & \textbf{0.3264 (6)} & 0.5827 (3)          & \textbf{0.4045 (5)} & 0.1125 (9)          & \textbf{0.8028 (1)} & \textbf{0.7889 (2)} \\
    18\_WPBC            & 0.4983 (3)      & 0.0799 (8)          & 0.2656 (7)          & 0.0313 (9)          & 0.4997 (2)          & 0.3385 (6)          & \textbf{0.4273 (5)} & 0.4399 (4)          & \textbf{0.7014 (1)} \\
    19\_annthyroid      & 0.5952 (8)      & 0.6528 (7)          & \textbf{0.7292 (3)} & 0.6667 (5)          & 0.5661 (9)          & 0.7743 (2)          & 0.6713 (4)          & \textbf{0.8278 (1)} & 0.6574 (6)          \\
    20\_arrhythmia      & 0.4706 (6)      & 0.3958 (7)          & 0.5399 (5)          & 0.0174 (9)          & 0.6879 (3)          & 0.6927 (2)          & 0.2664 (8)          & 0.5816 (4)          & \textbf{0.8564 (1)} \\
    21\_breastw         & 0.4152 (7)      & 0.599 (5)           & 0.7257 (2)          & 0.5104 (6)          & \textbf{0.8844 (1)} & 0.0556 (9)          & 0.6609 (3)          & 0.6003 (4)          & 0.4115 (8)          \\
    22\_glass           & 0.564 (5)       & 0.1684 (8)          & 0.75 (4)            & 0.0729 (9)          & 0.517 (6)           & \textbf{0.3524 (7)} & \textbf{0.9308 (1)} & 0.7594 (3)          & 0.9201 (2)          \\
    23\_ionosphere      & 0.3218 (5)      & 0.0451 (8)          & 0.1875 (6)          & \textbf{0.941 (1)}  & 0.4637 (4)          & 0.0694 (7)          & 0.0035 (9)          & 0.85 (3)            & \textbf{0.941 (1)}  \\
    24\_letter          & 0.4983 (6)      & 0.224 (7)           & 0.1354 (8)          & 0.7778 (4)          & 0.5384 (5)          & \textbf{0.9722 (1)} & 0.0104 (9)          & 0.7812 (3)          & 0.8201 (2)          \\
    25\_lympho          & 0.4152 (5)      & 0.0556 (9)          & 0.2951 (6)          & 0.6233 (4)          & 0.7772 (2)          & \textbf{0.8108 (1)} & 0.6522 (3)          & 0.2455 (7)          & \textbf{0.1597 (8)} \\
    26\_mammography     & 0.5502 (7)      & 0.6458 (4)          & \textbf{0.7361 (1)} & 0.5521 (6)          & 0.5356 (8)          & \textbf{0.6563 (3)} & 0.7076 (2)          & 0.5267 (9)          & 0.5536 (5)          \\
    27\_mnist           & 0.4187 (6)      & \textbf{0.1285 (8)} & 0.8507 (2)          & 0.2917 (7)          & 0.618 (5)           & 0.6302 (4)          & 0.0035 (9)          & 0.7674 (3)          & \textbf{0.9152 (1)} \\
    28\_musk            & 0.2595 (8)      & 0.9253 (2)          & \textbf{0.9253 (1)} & \textbf{0.3368 (7)} & 0.7661 (5)          & 0.066 (9)           & 0.8443 (4)          & 0.6722 (6)          & 0.9239 (3)          \\
    29\_optdigits       & 0.4879 (7)      & 0.6215 (4)          & 0.6597 (3)          & 0.4861 (8)          & 0.6118 (5)          & 0.7465 (2)          & \textbf{0.6003 (6)} & 0.4281 (9)          & \textbf{0.9325 (1)} \\
    30\_pendigits       & 0.526 (5)       & 0.0764 (9)          & 0.9826 (2)          & 0.3611 (7)          & \textbf{0.6893 (4)} & \textbf{1 (1)}      & 0.8166 (3)          & 0.2007 (8)          & 0.3837 (6)          \\
    31\_pima            & 0.3737 (7)      & 0.3802 (6)          & 0.4514 (4)          & \textbf{0.8628 (1)} & 0.609 (2)           & 0.5729 (3)          & 0.1246 (9)          & 0.4038 (5)          & \textbf{0.2535 (8)} \\
    32\_satellite       & 0.4533 (6)      & 0.9861 (2)          & 0.3247 (8)          & \textbf{0.2535 (9)} & 0.51 (5)            & 0.4063 (7)          & \textbf{0.9965 (1)} & 0.5608 (4)          & 0.7274 (3)          \\
    33\_satimage-2      & 0.436 (3)       & 0.3854 (5)          & 0.0069 (9)          & \textbf{0.4132 (4)} & \textbf{0.7848 (1)} & 0.5226 (2)          & 0.0138 (8)          & 0.266 (6)           & 0.191 (7)           \\
    34\_speech          & 0.6817 (3)      & 0.6458 (4)          & 0.5573 (5)          & 0.5573 (5)          & \textbf{0.9052 (1)} & 0.349 (7)           & 0.0069 (9)          & 0.259 (8)           & \textbf{0.7024 (2)} \\
    35\_thyroid         & 0.5294 (7)      & \textbf{0.9549 (1)} & 0.2309 (9)          & 0.8646 (3)          & \textbf{0.4976 (8)} & 0.5556 (6)          & 0.7197 (5)          & 0.7222 (4)          & 0.8819 (2)          \\
    36\_vertebral       & 0.6367 (7)      & 0.8333 (6)          & 0.9549 (3)          & 0.9757 (2)          & 0.3239 (8)          & 0.8715 (5)          & 0.0208 (9)          & \textbf{0.9125 (4)} & \textbf{0.9861 (1)} \\
    37\_vowels          & 0.5606 (4)      & 0.2639 (8)          & 0.3038 (7)          & \textbf{0.8785 (1)} & 0.6692 (3)          & 0.8403 (2)          & 0.0208 (9)          & 0.4854 (6)          & 0.5382 (5)          \\
    38\_wbc             & 0.4844 (6)      & \textbf{0.1389 (7)} & 0.559 (5)           & 0.1007 (8)          & 0.5599 (4)          & 0.7326 (3)          & \textbf{0.9308 (1)} & 0.8899 (2)          & 0.0313 (9)          \\
    39\_wine            & 0.5917 (4)      & \textbf{0.9063 (1)} & 0.059 (8)           & 0.0104 (9)          & 0.501 (6)           & \textbf{0.6806 (2)} & 0.5709 (5)          & 0.6031 (3)          & 0.3875 (7)          \\
    \midrule
    Average             & 0.4901 (7)      & 0.4598 (8)          & 0.5438 (5)          & 0.5113 (6)          & 0.5969 (3)          & \textbf{0.5615 (4)} & 0.4095 (9)          & 0.5981 (2)          & \textbf{0.6835 (1)} \\
    STD                 & 0.0960          & 0.3493              & 0.2904              & 0.3025              & 0.1364              & 0.2903              & 0.3613              & 0.2087              & 0.2790             \\
    \midrule
    Avg. Rank & 5.7179 &	5.6923&	4.7692&	5.3846&	4.5641	&4.5385	&6.0769&	4.6410&	\textbf{3.5128}
\\
    \bottomrule
    \end{tabular}
    }
    \caption{Method evaluation on iForest (normalized AP rank). The most performing method is highlighted in bold. The algo. rank is provided in parenthesis (lower ranks denote better performance). \method achieves the best performance among all.}
        \label{table:full_iforest_results}

\end{table*}

==> backup_aaai/tables/all_lof_results.tex <==
\begin{table*}[!ht]
    \footnotesize

    \scalebox{0.95}{
    \begin{tabular}{l|lllllll|ll}
    \toprule
    \textbf{datasets}   & \textbf{Random} & \textbf{GB}         & \textbf{ISAC}       & \textbf{AS}         & \textbf{HyperEns}   & \textbf{MetaOD}     & \textbf{Default}    & \textbf{HPOD\_0}    & \textbf{HPOD}       \\
    \midrule
1\_ALOI             & 0.6418 (5)      & 0.6825 (4)          & 0.625 (6)           & \textbf{0.95 (1)}  & 0.005 (9)           & 0.1319 (8)          & 0.905 (2)           & 0.8975 (3)          & \textbf{0.3433 (7)} \\
2\_Annthyroid       & 0.5224 (7)      & \textbf{0.6175 (5)} & 0.565 (6)           & 0.0275 (8)         & 0.8836 (3)          & 0.9236 (2)          & \textbf{0.97 (1)}   & 0.0125 (9)          & \textbf{0.6841 (4)} \\
3\_Arrhythmia       & 0.3134 (8)      & \textbf{0.4125 (5)} & 0.4 (6)             & \textbf{0.98 (1)}  & 0.8557 (3)          & 0.2188 (9)          & 0.335 (7)           & 0.92 (2)            & 0.7761 (4)          \\
4\_Cardiotocography & 0.4776 (4)      & 0.31 (6)            & \textbf{0.745 (3)}  & 0.19 (8)           & \textbf{1 (1)}      & 0.4583 (5)          & 0.165 (9)           & 0.2225 (7)          & \textbf{0.985 (2)}  \\
5\_Glass            & 0.5721 (3)      & 0.3975 (5)          & 0.725 (2)           & 0.02 (9)           & \textbf{0.2647 (7)} & 0.1684 (8)          & \textbf{0.95 (1)}   & 0.3525 (6)          & 0.5498 (4)          \\
6\_HeartDisease     & 0.5473 (6)      & 0.7625 (3)          & 0.4825 (7)          & 0.035 (9)          & \textbf{1 (1)}      & 0.6319 (4)          & 0.32 (8)            & 0.555 (5)           & \textbf{0.8507 (2)} \\
7\_InternetAds      & 0.5174 (5)      & 0.5675 (3)          & \textbf{1 (1)}      & 0.39 (7)           & \textbf{0.4825 (6)} & \textbf{0.9132 (2)} & 0.02 (9)            & 0.2775 (8)          & 0.5572 (4)          \\
8\_PageBlocks       & 0.4129 (6)      & 0.4425 (5)          & \textbf{0.985 (1)}  & \textbf{0.235 (8)} & 0.61 (3)            & 0.5903 (4)          & 0.24 (7)            & 0.155 (9)           & \textbf{0.8507 (2)} \\
9\_PenDigits        & 0.3333 (7)      & 0.3475 (6)          & 0.69 (4)            & \textbf{0.4 (5)}   & \textbf{0.1333 (8)} & 0.8924 (3)          & \textbf{0.9 (1)}    & 0.075 (9)           & \textbf{0.9 (1)}    \\
10\_Pima            & 0.3184 (8)      & 0.535 (6)           & \textbf{0.9975 (1)} & 0.47 (7)           & 0.99 (2)            & 0.783 (4)           & 0.02 (9)            & 0.59 (5)            & \textbf{0.9125 (3)} \\
11\_Shuttle         & 0.5174 (6)      & 0.2725 (8)          & 0.52 (5)            & 0.6925 (3)         & \textbf{0.0229 (9)} & 0.309 (7)           & \textbf{0.895 (1)}  & \textbf{0.7125 (2)} & 0.6925 (3)          \\
12\_SpamBase        & 0.403 (5)       & 0.4075 (4)          & 0.21 (6)            & \textbf{0.17 (8)}  & \textbf{1 (1)}      & 0.1823 (7)          & \textbf{0.155 (9)}  & 0.715 (3)           & 0.8259 (2)          \\
13\_Stamps          & 0.408 (4)       & 0.4225 (3)          & 0.8 (2)             & 0.08 (9)           & 0.408 (4)           & \textbf{0.1406 (8)} & 0.195 (6)           & 0.1625 (7)          & \textbf{0.815 (1)}  \\
14\_Waveform        & 0.7761 (3)      & 0.2025 (6)          & \textbf{0.3425 (5)} & 0.175 (7)          & 0.0338 (9)          & 0.6528 (4)          & 0.85 (2)            & \textbf{0.0575 (8)} & \textbf{0.975 (1)}  \\
15\_WBC             & 0.5522 (5)      & 0.4175 (6)          & \textbf{0.99 (1)}   & 0.01 (9)           & 0.9284 (3)          & \textbf{0.9653 (2)} & 0.195 (7)           & 0.1775 (8)          & 0.765 (4)           \\
16\_WDBC            & 0.1592 (8)      & 0.6575 (3)          & 0.755 (2)           & 0.6575 (3)         & 0.1095 (9)          & \textbf{0.8368 (1)} & 0.235 (6)           & 0.6575 (3)          & \textbf{0.2 (7)}    \\
17\_Wilt            & 0.4378 (4)      & 0.645 (3)           & \textbf{0.185 (7)}  & \textbf{1 (1)}     & 0.005 (9)           & \textbf{0.4045 (5)} & 0.2 (6)             & \textbf{0.995 (2)}  & \textbf{0.17 (8)}   \\
18\_WPBC            & 0.2886 (8)      & 0.695 (4)           & 0.7575 (2)          & 0.54 (6)           & 0.2527 (9)          & 0.3385 (7)          & \textbf{0.7275 (3)} & \textbf{0.95 (1)}   & \textbf{0.615 (5)}  \\
19\_annthyroid      & 0.4428 (8)      & 0.2525 (9)          & \textbf{0.58 (6)}   & \textbf{1 (1)}     & 0.9343 (2)          & 0.7743 (3)          & 0.485 (7)           & \textbf{0.61 (5)}   & 0.7475 (4)          \\
20\_arrhythmia      & 0.4328 (6)      & 0.4425 (5)          & 0.165 (9)           & 0.94 (2)           & 0.7055 (3)          & 0.6927 (4)          & 0.205 (7)           & 0.19 (8)            & \textbf{0.99 (1)}   \\
21\_breastw         & 0.6318 (6)      & 0.0975 (8)          & 0.8 (3)             & 0.7025 (4)         & \textbf{1 (1)}      & 0.0556 (9)          & 0.185 (7)           & 0.8675 (2)          & 0.7025 (4)          \\
22\_glass           & 0.5473 (3)      & 0.5175 (4)          & 0.105 (8)           & 0.325 (7)          & 0.0229 (9)          & \textbf{0.3524 (6)} & \textbf{0.91 (2)}   & \textbf{0.9825 (1)} & 0.4428 (5)          \\
23\_ionosphere      & 0.3781 (5)      & 0.5125 (4)          & \textbf{0.985 (1)}  & \textbf{0.77 (3)}  & 0.205 (7)           & 0.0694 (8)          & 0.055 (9)           & 0.2825 (6)          & \textbf{0.9403 (2)} \\
24\_letter          & 0.5224 (5)      & 0.7425 (3)          & 0.055 (7)           & 0.005 (8)          & 0.005 (9)           & \textbf{0.9722 (1)} & 0.95 (2)            & 0.44 (6)            & 0.54 (4)            \\
25\_lympho          & 0.4428 (6)      & 0.8275 (2)          & 0.03 (9)            & 0.3 (7)            & \textbf{0.9721 (1)} & \textbf{0.8108 (3)} & 0.6375 (5)          & 0.2425 (8)          & \textbf{0.805 (4)}  \\
26\_mammography     & 0.4129 (6)      & 0.4175 (5)          & \textbf{0.9075 (2)} & 0.215 (7)          & \textbf{1 (1)}      & \textbf{0.6563 (4)} & 0.045 (9)           & 0.1825 (8)          & 0.6775 (3)          \\
27\_mnist           & 0.5025 (5)      & \textbf{0.4175 (6)} & 0.24 (8)            & 0.055 (9)          & 0.7522 (2)          & 0.6302 (3)          & 0.505 (4)           & 0.405 (7)           & \textbf{0.79 (1)}   \\
28\_musk            & 0.7662 (2)      & 0.6475 (4)          & \textbf{0.59 (5)}   & \textbf{0.155 (8)} & \textbf{1 (1)}      & 0.066 (9)           & 0.675 (3)           & 0.3575 (7)          & 0.3881 (6)          \\
29\_optdigits       & 0.5572 (7)      & 0.8925 (3)          & 0.3225 (9)          & \textbf{1 (1)}     & 0.6299 (6)          & 0.7465 (5)          & \textbf{0.765 (4)}  & 0.905 (2)           & \textbf{0.45 (8)}   \\
30\_pendigits       & 0.6219 (8)      & 0.6625 (6)          & 0.6275 (7)          & 0.1725 (9)         & \textbf{1 (1)}      & \textbf{1 (1)}      & 0.675 (5)           & 0.7525 (4)          & 0.77 (3)            \\
31\_pima            & 0.4776 (6)      & 0.4225 (7)          & \textbf{0.9525 (1)} & \textbf{0.92 (2)}  & 0.3775 (8)          & 0.5729 (5)          & 0.05 (9)            & 0.8875 (3)          & \textbf{0.86 (4)}   \\
32\_satellite       & 0.408 (4)       & 0.2725 (8)          & 0.36 (7)            & \textbf{0.905 (3)} & \textbf{1 (1)}      & 0.4063 (5)          & \textbf{0.25 (9)}   & 0.365 (6)           & 0.985 (2)           \\
33\_satimage-2      & 0.5771 (6)      & 0.3325 (8)          & 0.7725 (5)          & \textbf{0.98 (1)}  & \textbf{0.855 (4)}  & 0.5226 (7)          & 0.94 (2)            & 0.915 (3)           & 0.005 (9)           \\
34\_speech          & 0.8209 (3)      & 0.8275 (2)          & 0.57 (5)            & 0.3275 (8)         & \textbf{0.8945 (1)} & 0.349 (7)           & 0.025 (9)           & 0.42 (6)            & \textbf{0.6825 (4)} \\
35\_thyroid         & 0.4925 (7)      & \textbf{0.2925 (8)} & 0.925 (3)           & \textbf{1 (1)}     & \textbf{0.999 (2)}  & 0.5556 (6)          & 0.24 (9)            & 0.58 (5)            & 0.91 (4)            \\
36\_vertebral       & 0.3881 (6)      & 0.6975 (4)          & 0.045 (9)           & 0.135 (8)          & 0.2418 (7)          & 0.8715 (2)          & 0.7375 (3)          & \textbf{0.885 (1)}  & \textbf{0.49 (5)}   \\
37\_vowels          & 0.403 (5)       & 0.2875 (7)          & 0.385 (6)           & \textbf{0.63 (3)}  & 0.0259 (9)          & 0.8403 (2)          & 0.055 (8)           & 0.515 (4)           & \textbf{0.9652 (1)} \\
38\_wbc             & 0.3731 (6)      & \textbf{0.5575 (4)} & 0.435 (5)           & 0.19 (9)           & \textbf{0.9771 (1)} & 0.7326 (3)          & \textbf{0.2 (8)}    & 0.32 (7)            & 0.9478 (2)          \\
39\_wine            & 0.3632 (5)      & \textbf{0.5875 (2)} & 0.44 (4)            & 0.055 (8)          & 0.1512 (7)          & \textbf{0.6806 (1)} & 0.21 (6)            & 0.0425 (9)          & 0.5275 (3)          \\
\bottomrule
Average             & 0.4811 (7)      & 0.5001 (6)          & 0.5658 (3)          & 0.4565 (8)         & 0.5829 (2)          & \textbf{0.5615 (4)} & 0.4379 (9)          & 0.5034 (5)          & \textbf{0.6945 (1)} \\
STD                 & 0.1354          & 0.1911              & 0.3005              & 0.3659             & 0.3996              & 0.2903              & 0.3397              & 0.3122              & 0.2457              \\
    \midrule
    Avg. Rank & 5.5641&	4.9744	&4.7692&	5.5897&	4.5897	&4.7179	&5.6667	&5.2564	&\textbf{3.6667}

\\
    \bottomrule
    \end{tabular}
    }
    \caption{Method evaluation on LOF (normalized AP rank). The most performing method is highlighted in bold. The algo. rank is provided in parenthesis (lower ranks denote better performance). \method achieves the best performance among all baselines.}
        \label{table:full_lof_results}

\end{table*}

==> backup_aaai/tables/all_rae_results.tex <==
\begin{table*}[!ht]
    \footnotesize

    \scalebox{0.95}{
    \begin{tabular}{l|lllllll|ll}
    \toprule
    \textbf{datasets}   & \textbf{Random} & \textbf{GB}         & \textbf{ISAC}       & \textbf{AS}         & \textbf{HyperEns}   & \textbf{MetaOD}     & \textbf{MinLoss}    & \textbf{HPOD\_0}    & \textbf{HPOD}       \\
    \midrule
    1\_ALOI             & 0.8234 (3)      & 0.6445 (4)          & 0.6445 (4)          & 0.0612 (8)          & 0.6286 (6)          & 0.0612 (8)          & 0.3747 (7)          & 0.9206 (2)          & \textbf{0.974 (1)}  \\
    2\_Annthyroid       & 0.5506 (5)      & 0.0404 (9)          & 0.4336 (6)          & 0.5508 (4)          & 0.2499 (8)          & 0.8659 (2)          & 0.5651 (3)          & 0.3211 (7)          & \textbf{0.9883 (1)} \\
    3\_Arrhythmia       & 0.4688 (9)      & 0.8112 (5)          & 0.7435 (6)          & \textbf{0.9987 (1)} & 0.4836 (8)          & 0.9036 (3)          & 0.7013 (7)          & 0.9451 (2)          & 0.9036 (3)          \\
    4\_Cardiotocography & 0.6519 (5)      & 0.5951 (6)          & 0.819 (3)           & 0.1432 (9)          & 0.6727 (4)          & 0.2786 (8)          & 0.5544 (7)          & 0.949 (2)           & \textbf{0.9688 (1)} \\
    5\_Glass            & 0.6403 (3)      & 0.5781 (6)          & 0.4036 (7)          & 0.1823 (9)          & \textbf{0.7065 (1)} & 0.6094 (5)          & 0.2651 (8)          & 0.6549 (2)          & 0.6354 (4)          \\
    6\_HeartDisease     & 0.5156 (3)      & 0.3958 (6)          & 0.5156 (2)          & 0.056 (8)           & \textbf{0.5662 (1)} & 0.1901 (7)          & 0.4128 (5)          & 0.4487 (4)          & 0.056 (8)           \\
    7\_InternetAds      & 0.6623 (2)      & 0.5156 (7)          & 0.5156 (7)          & 0.5221 (6)          & \textbf{0.6743 (1)} & 0.5404 (5)          & 0.3419 (9)          & 0.6549 (3)          & 0.651 (4)           \\
    8\_PageBlocks       & 0.7584 (5)      & 0.7591 (3)          & 0.7591 (3)          & \textbf{0.9779 (1)} & 0.6078 (7)          & 0.3047 (8)          & 0.7544 (6)          & 0.3047 (8)          & 0.9505 (2)          \\
    9\_PenDigits        & 0.4909 (4)      & 0.0391 (9)          & 0.1289 (7)          & 0.4909 (5)          & \textbf{0.8 (1)}    & 0.4909 (5)          & 0.5247 (3)          & 0.619 (2)           & 0.1289 (7)          \\
    10\_Pima            & 0.4117 (8)      & 0.8698 (3)          & 0.8698 (3)          & 0.9779 (1)          & 0.7792 (5)          & 0.4115 (9)          & 0.6865 (6)          & 0.5247 (7)          & \textbf{0.9779 (1)} \\
    11\_Shuttle         & 0.3195 (2)      & 0.319 (3)           & 0.319 (3)           & 0.319 (3)           & \textbf{0.3849 (1)} & 0.319 (3)           & 0.2464 (7)          & 0.0784 (8)          & 0.056 (9)           \\
    12\_SpamBase        & 0.3208 (6)      & 0.1276 (8)          & 0.1276 (8)          & \textbf{0.9323 (1)} & 0.4618 (4)          & 0.7214 (2)          & 0.5242 (3)          & 0.194 (7)           & 0.3364 (5)          \\
    13\_Stamps          & 0.6727 (5)      & 0.6302 (6)          & 0.1133 (9)          & 0.5924 (7)          & 0.7777 (4)          & \textbf{0.9844 (1)} & 0.5318 (8)          & 0.9026 (3)          & 0.9714 (2)          \\
    14\_Waveform        & 0.687 (8)       & 0.7018 (7)          & 0.8242 (5)          & 0.8932 (2)          & 0.5257 (9)          & 0.8932 (2)          & 0.7977 (6)          & \textbf{0.9513 (1)} & 0.8932 (2)          \\
    15\_WBC             & 0.3403 (4)      & 0.3398 (5)          & \textbf{0.8242 (1)} & 0.1628 (8)          & 0.6966 (2)          & 0.6328 (3)          & 0.0648 (9)          & 0.2628 (6)          & 0.2435 (7)          \\
    16\_WDBC            & 0.5896 (5)      & 0.3542 (7)          & 0.0378 (9)          & 0.9115 (2)          & 0.5849 (6)          & 0.3542 (7)          & 0.7099 (4)          & 0.7219 (3)          & \textbf{0.9935 (1)} \\
    17\_Wilt            & 0.5013 (8)      & 0.5013 (1)          & \textbf{0.5013 (1)} & \textbf{0.5013 (1)} & 0.0026 (9)          & \textbf{0.5013 (1)} & 0.5013 (1)          & \textbf{0.5013 (1)} & \textbf{0.5013 (1)} \\
    18\_WPBC            & 0.5039 (5)      & 0.2943 (8)          & 0.5846 (4)          & 0.737 (2)           & 0.2899 (9)          & 0.6354 (3)          & \textbf{0.7562 (1)} & 0.4445 (7)          & 0.5039 (5)          \\
    19\_annthyroid      & 0.6351 (7)      & 0.3112 (8)          & \textbf{0.9922 (1)} & 0.9701 (2)          & 0.8379 (5)          & 0.8307 (6)          & 0.131 (9)           & 0.8703 (4)          & 0.9312 (3)          \\
    20\_arrhythmia      & 0.4753 (9)      & 0.6432 (7)          & 0.9714 (2)          & 0.9596 (4)          & 0.5143 (8)          & 0.7344 (5)          & 0.6883 (6)          & 0.969 (3)           & \textbf{0.9844 (1)} \\
    21\_breastw         & 0.139 (6)       & 0.0716 (9)          & 0.6719 (2)          & 0.138 (7)           & \textbf{0.9818 (1)} & 0.138 (7)           & 0.2052 (5)          & 0.6719 (2)          & 0.6714 (4)          \\
    22\_glass           & 0.4584 (6)      & 0.6589 (3)          & 0.6693 (2)          & 0.375 (8)           & 0.5475 (4)          & \textbf{0.7865 (1)} & 0.1318 (9)          & 0.3802 (7)          & 0.5312 (5)          \\
    23\_ionosphere      & 0.7039 (9)      & 0.8047 (6)          & 0.8216 (5)          & \textbf{0.9844 (1)} & 0.7143 (8)          & 0.7969 (7)          & 0.8307 (4)          & 0.9096 (3)          & 0.9351 (2)          \\
    24\_letter          & 0.5013 (3)      & 0.0872 (7)          & 0.0182 (8)          & 0.0182 (8)          & 0.5273 (2)          & \textbf{0.918 (1)}  & 0.4492 (4)          & 0.1643 (6)          & 0.2591 (5)          \\
    25\_lympho          & 0.7506 (8)      & 0.7695 (7)          & 0.8802 (5)          & 0.9583 (3)          & 0.6545 (9)          & 0.974 (2)           & 0.7805 (6)          & 0.9177 (4)          & \textbf{1 (1)}      \\
    26\_mammography     & 0.4844 (6)      & 0.3607 (9)          & 0.4844 (7)          & 0.3841 (8)          & 0.5896 (4)          & \textbf{0.9349 (1)} & 0.7328 (3)          & 0.531 (5)           & 0.7865 (2)          \\
    27\_mnist           & 0.6052 (6)      & \textbf{0.9818 (1)} & 0.7786 (3)          & 0.2513 (9)          & 0.5496 (7)          & 0.6406 (5)          & 0.4677 (8)          & 0.7279 (4)          & 0.9401 (2)          \\
    28\_musk            & 0.5584 (8)      & 0.901 (2)           & 0.6289 (6)          & \textbf{0.9857 (1)} & 0.5922 (7)          & 0.7018 (5)          & 0.1414 (9)          & 0.8112 (4)          & 0.8516 (3)          \\
    29\_optdigits       & 0.5286 (5)      & 0.1406 (8)          & 0.5977 (3)          & 0.2122 (7)          & 0.6509 (2)          & 0.5977 (3)          & \textbf{0.794 (1)}  & 0.2721 (6)          & 0.0755 (9)          \\
    30\_pendigits       & 0.626 (3)       & 0.5169 (6)          & 0.5299 (5)          & 0.1445 (8)          & \textbf{0.8119 (1)} & 0.0924 (9)          & 0.318 (7)           & 0.7096 (2)          & 0.613 (4)           \\
    31\_pima            & 0.713 (4)       & 0.7135 (3)          & 0.569 (7)           & 0.569 (7)           & 0.6312 (6)          & 0.569 (7)           & 0.6779 (5)          & 0.9247 (2)          & \textbf{0.9987 (1)} \\
    32\_satellite       & 0.8714 (4)      & 0.8503 (6)          & 0.8685 (5)          & \textbf{0.9909 (1)} & 0.7813 (7)          & 0.2865 (9)          & 0.7471 (8)          & 0.9471 (2)          & 0.9323 (3)          \\
    33\_satimage-2      & 0.9143 (3)      & 0.8333 (6)          & 0.8737 (5)          & \textbf{0.987 (1)}  & 0.7927 (7)          & 0.3997 (9)          & 0.481 (8)           & 0.9063 (4)          & 0.9506 (2)          \\
    34\_speech          & 0.6299 (7)      & 0.9714 (3)          & 0.4154 (9)          & 0.9792 (2)          & 0.4842 (8)          & 0.8177 (4)          & 0.6773 (6)          & 0.699 (5)           & \textbf{0.9909 (1)} \\
    35\_thyroid         & 0.6468 (8)      & 0.9245 (4)          & 0.8633 (6)          & 0.9453 (2)          & \textbf{0.9647 (1)} & 0.7305 (7)          & 0.2867 (9)          & 0.9164 (5)          & 0.9247 (3)          \\
    36\_vertebral       & 0.6974 (8)      & 0.6979 (3)          & 0.6979 (3)          & 0.6979 (3)          & 0.4649 (9)          & 0.6979 (3)          & 0.7487 (2)          & \textbf{0.8133 (1)} & 0.6979 (3)          \\
    37\_vowels          & 0.7506 (7)      & 0.9349 (4)          & 0.4648 (9)          & \textbf{0.9974 (1)} & 0.6987 (8)          & 0.8581 (6)          & 0.869 (5)           & 0.9846 (2)          & 0.9818 (3)          \\
    38\_wbc             & 0.6195 (6)      & \textbf{0.9401 (1)} & 0.8815 (3)          & 0.5443 (7)          & 0.6566 (5)          & 0.5443 (7)          & 0.456 (9)           & 0.9117 (2)          & 0.8727 (4)          \\
    39\_wine            & 0.4818 (4)      & 0.4818 (5)          & 0.4818 (5)          & 0.4818 (5)          & 0.9403 (2)          & \textbf{0.9714 (1)} & 0.5797 (3)          & 0.387 (9)           & 0.4818 (5)          \\
    \midrule
    Average             & 0.5821 (7)      & 0.567 (8)           & 0.5981 (6)          & 0.6047 (5)          & 0.6226 (3)          & \textbf{0.6082 (4)} & 0.5258 (9)          & 0.6622 (2)          & \textbf{0.7216 (1)} \\
    STD                 & 0.1580          & 0.2884              & 0.2630              & 0.3478              & 0.1937              & 0.2647              & 0.2261              & 0.2718              & 0.3103             \\
    \midrule
    Avg. Rank & 5.5641&	5.4103&	4.8462&	4.4359&	5.0513&	4.7949	&5.7949	&4.0256&	\textbf{3.3333}
 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Method evaluation on RAE (normalized AP rank). The most performing method is highlighted in bold. The algo. rank is provided in parenthesis (lower ranks denote better performance). \method achieves the best performance among all baselines.}    \label{table:full_rae_results}

\end{table*}

==> backup_aaai/tables/baseline.tex <==
\setlength\tabcolsep{1.5 pt}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\begin{table}[!h]
\vspace{-0.1in}
\centering
\scalebox{0.64}{
\begin{tabular}{l|ccc|ccccc|cc}
\toprule
\textbf{Category}      & \textbf{Default} & \textbf{Random} & \textbf{MinLoss} & \textbf{HE} & \textbf{GB} & \textbf{ISAC} & \textbf{AS} & \textbf{MetaOD} &  \textbf{\methodz} & \method \\
\midrule
\textbf{meta-learning} &    \xmark &    \xmark            &   \xmark        &  \xmark        &        \cmark  &          \cmark    &           \cmark &     \cmark & \textcolor{dodgerblue}{\cmark} & \textcolor{dodgerblue}{\cmark} \\ 
\midrule
% \textbf{HPO} &       \xmark          &     \xmark &    \cmark     &  \xmark        &        \cmark  &          \cmark    &           \cmark &     \cmark & \textcolor{dodgerblue}{\cmark} & \textcolor{dodgerblue}{\cmark}\\ 
\textbf{discrete HP} &         \xmark     &    \xmark   &       \cmark    &      \xmark    &        \cmark  &          \cmark    &           \cmark &     \cmark & \textcolor{dodgerblue}{\cmark} & \textcolor{dodgerblue}{\cmark}     \\ 
\textbf{continuous HP} &       \xmark   &    \xmark       &  \cmark         &      \xmark    &       \xmark   &     \xmark         &      \xmark      & \xmark& \textcolor{dodgerblue}{\cmark} & \textcolor{dodgerblue}{\cmark}     \\ 

\bottomrule
\end{tabular}
}
\vspace{-0.1in}
	\caption{\method and baselines for comparison with categorization by (first row) whether it uses meta-learning 
 % (second row) whether it is an HPO method 
 and (second \& third row) whether it supports \textit{discrete} and \textit{continuous} HPO. Only \method and 
 % its variant 
 \methodz leverage meta-learning and support continuous HPO.
 % Only MinLoss and \method (and its variant \methodz) support continuous HPO. 
 See details in \S \ref{subsec:exp_details}.
 % See additional details of baselines in \S \ref{subsec:exp_details}.
 } % title of Table
% 	\footnotesize
\vspace{-0.1in}
	\label{table:baseline} % is used to refer this table in the text
	\vspace{-0.15in}
\end{table}
\setlength\tabcolsep{6 pt}

==> backup_aaai/tables/case_study.tex <==
\begin{table}[!htb]
\centering
	\vspace{-0.05in}
	\footnotesize
	
\scalebox{0.82}{
\begin{tabular}{l|ll|l}
\toprule
\textbf{\# Iter} & \textbf{Dist. metric} & \textbf{\# Neighbors} & \textbf{AP Value} \\
\midrule
1                & Manhattan         & 23                    & 0.2866                       \\
$\ldots$ &$\ldots$&$\ldots$&$\ldots$\\
6                & Cosine         & 42                    & 0.327                       \\
$\ldots$ &$\ldots$&$\ldots$&$\ldots$\\
10               & Cosine           & 55                    & 0.3438                       \\
$\ldots$ &$\ldots$&$\ldots$&$\ldots$\\
20               & Chebyshev        & 72                    & 0.3569                      \\
$\ldots$ &$\ldots$&$\ldots$&$\ldots$\\
30               & Chebyshev        & 73                    & 0.357                       \\
\midrule\midrule
\textbf{Optimal} & Chebyshev        & 79                    & \textbf{0.3609}                  \\
\bottomrule          
\end{tabular}
}\vspace{-0.05in}
	\caption{Trace of \method on \texttt{Cardiotocography} dataset. Over iterations (col. 1), \method gradually identifies better HPs (col. 2 \&3), with higher AP (col. 4). The optimal HP on from the meta-HP set is \{'Chebyshev', 79\}, which \method gets closer to the optimal HP during its adaptive search.} % title of Table
	\label{table:case_study} % is used to refer this table in the text
	\vspace{-0.05in}
\end{table}

==> backup_aaai/tables/case_study_full.tex <==
\begin{table}[!ht]
\centering
% 	\vspace{-0.1in}
	\footnotesize
	
\scalebox{1}{
\begin{tabular}{l|ll|l}
\toprule
\textbf{\# Iter} & \textbf{Metrics} & \textbf{\# Neighbors} & \textbf{Norm. AP Rank} \\
\midrule
1                & Manhattan         & 23                    & 0.2866          \\
2                & Manhattan         & 23                    & 0.2866          \\
3                & Manhattan         & 23                    & 0.2866          \\
4                & Manhattan         & 23                    & 0.2866          \\
5                & Cosine           & 41                    & 0.327           \\
6                & Cosine           & 42                    & 0.327           \\
7                & Cosine           & 55                    & 0.3438          \\
8                & Cosine           & 55                    & 0.3438          \\
9                & Cosine           & 55                    & 0.3438          \\
10               & Cosine           & 55                    & 0.3438          \\
11               & Cosine           & 55                    & 0.3438          \\
12               & Cosine           & 55                    & 0.3438          \\
13               & Cosine           & 55                    & 0.3438          \\
14               & Chebyshev        & 72                    & 0.3569          \\
15               & Chebyshev        & 72                    & 0.3569          \\
16               & Chebyshev        & 72                    & 0.3569          \\
17               & Chebyshev        & 72                    & 0.3569          \\
18               & Chebyshev        & 72                    & 0.3569          \\
19               & Chebyshev        & 72                    & 0.3569          \\
20               & Chebyshev        & 72                    & 0.3569          \\
21               & Chebyshev        & 72                    & 0.3569          \\
22               & Chebyshev        & 73                    & 0.357           \\
23               & Chebyshev        & 73                    & 0.357           \\
24               & Chebyshev        & 73                    & 0.357           \\
25               & Chebyshev        & 73                    & 0.357           \\
26               & Chebyshev        & 73                    & 0.357           \\
27               & Chebyshev        & 73                    & 0.357           \\
28               & Chebyshev        & 73                    & 0.357           \\
29               & Chebyshev        & 73                    & 0.357           \\
30               & Chebyshev        & 73                    & 0.357           \\
31               & Chebyshev        & 73                    & 0.357           \\
32               & Chebyshev        & 73                    & 0.357           \\
33               & Chebyshev        & 73                    & 0.357           \\
34               & Chebyshev        & 73                    & 0.357           \\
35               & Chebyshev        & 73                    & 0.357           \\
36               & Chebyshev        & 73                    & 0.357           \\
37               & Chebyshev        & 73                    & 0.357           \\
38               & Chebyshev        & 73                    & 0.357           \\
39               & Chebyshev        & 73                    & 0.357           \\
40               & Chebyshev        & 73                    & 0.357           \\
41               & Chebyshev        & 73                    & 0.357           \\
42               & Chebyshev        & 73                    & 0.357           \\
43               & Chebyshev        & 73                    & 0.357           \\
44               & Chebyshev        & 73                    & 0.357           \\
45               & Chebyshev        & 73                    & 0.357           \\
46               & Chebyshev        & 73                    & 0.357           \\
47               & Chebyshev        & 73                    & 0.357           \\
48               & Chebyshev        & 73                    & 0.357           \\
49               & Chebyshev        & 73                    & 0.357           \\
50               & Chebyshev        & 73                    & 0.357           \\
\midrule\midrule
\textbf{Optimal} & Chebyshev        & 79                    & \textbf{0.3609}                  \\
\bottomrule          
\end{tabular}
}
\caption{Full trace of \method on \texttt{Cardiotocography} dataset. Over iterations (col. 1), \method gradually identifies better HPs (col. 2 \&3), with higher AP (col. 4). The optimal HP on from the meta-HP set is \{'Chebyshev', 79\}, which \method gets closer to the optimal HP during its adaptive search (i.e., finding \{'Chebyshev', 73\} in 30 iterations).} % title of Table
	\label{table:case_study_full} % is used to refer this table in the text
	% \vspace{-0.15in}
\end{table}

==> backup_aaai/tables/datasets.tex <==
\begin{table}[!ht]
\centering
% 	\footnotesize
\scalebox{0.85}{
\begin{tabular}{ll|lll}
\toprule
\textbf{Dataset}   & \textbf{Source} & \textbf{\#Samples} & \textbf{\#Dims} & \textbf{\%Outlier} \\
\midrule
1\_ALOI             & DAMI            & 49534             & 27             & 3.04              \\
2\_Annthyroid       & DAMI            & 7129              & 21             & 7.49              \\
3\_Arrhythmia       & DAMI            & 450               & 259            & 45.78             \\
4\_Cardiotocography & DAMI            & 2114              & 21             & 22.04             \\
5\_Glass            & DAMI            & 214               & 7              & 4.21              \\
6\_HeartDisease     & DAMI            & 270               & 13             & 44.44             \\
7\_InternetAds      & DAMI            & 1966              & 1555           & 18.72             \\
8\_PageBlocks       & DAMI            & 5393              & 10             & 9.46              \\
9\_PenDigits        & DAMI            & 9868              & 16             & 0.2               \\
10\_Pima            & DAMI            & 768               & 8              & 34.9              \\
11\_Shuttle         & DAMI            & 1013              & 9              & 1.28              \\
12\_SpamBase        & DAMI            & 4207              & 57             & 39.91             \\
13\_Stamps          & DAMI            & 340               & 9              & 9.12              \\
14\_Waveform        & DAMI            & 3443              & 21             & 2.9               \\
15\_WBC             & DAMI            & 223               & 9              & 4.48              \\
16\_WDBC            & DAMI            & 367               & 30             & 2.72              \\
17\_Wilt            & DAMI            & 4819              & 5              & 5.33              \\
18\_WPBC            & DAMI            & 198               & 33             & 23.74             \\
\midrule
19\_annthyroid      & ODDS            & 7200              & 6              & 7.42              \\
20\_arrhythmia      & ODDS            & 452               & 274            & 14.6              \\
21\_breastw         & ODDS            & 683               & 9              & 34.99             \\
22\_glass           & ODDS            & 214               & 9              & 4.21              \\
23\_ionosphere      & ODDS            & 351               & 33             & 35.9              \\
24\_letter          & ODDS            & 1600              & 32             & 6.25              \\
25\_lympho          & ODDS            & 148               & 18             & 4.05              \\
26\_mammography     & ODDS            & 11183             & 6              & 2.32              \\
27\_mnist           & ODDS            & 7603              & 100            & 9.21              \\
28\_musk            & ODDS            & 3062              & 166            & 3.17              \\
29\_optdigits       & ODDS            & 5216              & 64             & 2.88              \\
30\_pendigits       & ODDS            & 6870              & 16             & 2.27              \\
31\_pima            & ODDS            & 768               & 8              & 34.9              \\
32\_satellite       & ODDS            & 6435              & 36             & 31.64             \\
33\_satimage-2      & ODDS            & 5803              & 36             & 1.22              \\
34\_speech          & ODDS            & 3686              & 400            & 1.65              \\
35\_thyroid         & ODDS            & 3772              & 6              & 2.47              \\
36\_vertebral       & ODDS            & 240               & 6              & 12.5              \\
37\_vowels          & ODDS            & 1456              & 12             & 3.43              \\
38\_wbc             & ODDS            & 378               & 30             & 5.56              \\
39\_wine            & ODDS            & 129               & 13             & 7.75             \\
\bottomrule
\end{tabular}
}

	\caption{Testbed composed by 18 datasets from DAMI library \cite{Campos2016evaluation} and 21 datasets from ODDS library \cite{Rayana2016b}.} % title of Table
 	\label{table:datasets} % is used to refer this table in the text
\vspace{-0.2in}
\end{table}
% \setlength\tabcolsep{6 pt}


==> backup_aaai/tables/hp_spaces.tex <==
\begin{table*}[!ht]
\centering
    % \footnotesize    
    \begin{subtable}[t]{\textwidth}
        \centering
        \caption{Key HPs optimized by \method for RAE. Both meta-HP set and inner-HP set include $2\times 3 \times 2 \times 2 \times 2 \times 2 \times 3 $=388 HP settings.}\label{table:rae_hps}

            \scalebox{1}{

        \begin{tabular}{l|ll|ll}
        \toprule
        & \textbf{HP Name} & \textbf{Type}      & \textbf{Meta-HP Set} & \textbf{Inner-HP Set}\\
        \midrule
       1 & \# EncodeLayers   & int (continuous)   & \{2,4\} & \{2,4\}              \\
       2 & Lambda           & float (continuous) & \{5e-5, 5e-3, 5e-1\} & \{1e-4, 1e-3, 1e-1\} \\
       3 &    Learning Rate    & float (continuous) & \{1e-3, 1e-2\}    & \{1e-3, 1e-2\}   \\
       4 &    \# Inner Epochs  & int (continuous)   & \{20, 50\}    & \{30, 40\}       \\
       5 &    \# Outer Epochs  & int (continuous)   & \{20, 50\}    & \{30, 40\}       \\
      6 &    Shrinkage Decay  & int (continuous)   & \{2,4\}        & \{2,4\}      \\
    7 &    Dropout          & float (continuous) & \{0, 0.1, 0.3, 0.5\} 
    & \{0, 0.1, 0.2, 0.4\}    \\
        \bottomrule
        \end{tabular}
    }
    \end{subtable}
    \vspace{0.1in}

    
    \begin{subtable}[t]{\textwidth}
        \centering
        \caption{Key HPs optimized by \method for LOF. Both meta-HP set and inner-HP set include $40\times 5$=200 HP settings.}\label{table:rae_lof}

            \scalebox{0.835}{

        \begin{tabular}{l|ll|ll}
        \toprule
        & \textbf{HP Name} & \textbf{Type}      & \textbf{Meta-HP Set} & \textbf{Inner-HP Set}\\
        \midrule
       1 & n\_neighbors     & int (continuous)  & \{1,3,5,$\dots$,80\} & \{2,4,6,$\dots$,81\}                                           \\
2 & distance metric           & str (categorical) &  \makecell{\{'chebyshev', 'minkowski', 'cosine', 'euclidean','manhattan'\}} & Same
        \\
        \bottomrule
        \end{tabular}
    }
    \end{subtable}
        \vspace{0.1in}


    \begin{subtable}[t]{\textwidth}
        \centering
        \caption{Key HPs optimized by \method for iForest. Both meta-HP set and inner-HP set include $8\times 9 \times 4$=288 HP settings.}\label{table:rae_iforest}

            \scalebox{0.98}{

        \begin{tabular}{l|ll|ll}
        \toprule
        & \textbf{HP Name} & \textbf{Type}      & \textbf{Meta-HP Set} & \textbf{Inner-HP Set}\\
        \midrule
       1&n\_estimators    & int (continuous)   & \{10,20,30,40,50,75,100,150\} & \{10,20,30,40,50,75,100,150\} \\
2&max\_samples     & float (continuous) & \{0.1, 0.2, $\dots$, 0.9\} & \{0.1, 0.2, $\dots$, 0.9\}            \\
3&max\_features    & float (continuous) & \{0.2, 0.4, 0.6, 0.8\} & \{0.3, 0.5, 0.7, 0.75\}        
        \\
        \bottomrule
        \end{tabular}
    }
    \end{subtable}
    \caption{Key HPs optimized by \method, and the meta-HP set and the inner-HP set used in this study.}
    \label{table:all_hps}
\end{table*}

==> backup_aaai/tables/iforest_pairs.tex <==
\begin{table}[h]
% \scriptsize
\caption{
Pairwise statistical test results between \method and baselines by Wilcoxon signed rank test. Statistically better method shown in \textbf{bold} (both marked \textbf{bold} if no significance).
For HPO on iForest, \method is statistically better than all, including the \textit{default} HP setting.}\label{table:iforest_pairs}
 \vspace{-0.1in}
\scalebox{0.87}{
\begin{tabular}{lll|lll}
\toprule
\textbf{Ours} & \textbf{Baseline} & \textbf{p-value} & \textbf{Ours} & \textbf{Baseline} & \textbf{p-value} \\
\midrule
\textbf{HPOD} & AS                & 0.0055           & \textbf{HPOD} & ISAC              & 0.0088           \\
\textbf{HPOD} & Random            & 0.0003           & \textbf{HPOD} & MetaOD            & 0.0289           \\
\textbf{HPOD} & \textbf{HyperEns} & 0.0484           & \textbf{HPOD} & ES                & 0.003            \\
\textbf{HPOD} & GB                & 0.0027           & \textbf{HPOD} & Default           & 0.0013               \\
\bottomrule
\end{tabular}}
% \vspace{0.05in}
\end{table}

==> backup_aaai/tables/lof_pairs.tex <==
\begin{table}[h]
% \scriptsize
\caption{
Pairwise statistical test results between \method and baselines by Wilcoxon signed rank test. Statistically better method shown in \textbf{bold} (both marked \textbf{bold} if no significance).
For HPO on LOF, \method is statistically better than all (except HyperEnsemble), including the \textit{default} HP setting.}\label{table:lof_pairs}
 \vspace{-0.1in}
\scalebox{0.87}{
\begin{tabular}{lll|lll}
\toprule
\textbf{Ours} & \textbf{Baseline} & \textbf{p-value} & \textbf{Ours} & \textbf{Baseline} & \textbf{p-value} \\
\midrule
\textbf{HPOD} & AS                & 0.0023           & \textbf{HPOD} & ISAC              & 0.0246           \\
\textbf{HPOD} & Random            & 0.0001           & \textbf{HPOD} & MetaOD            & 0.0088           \\
\textbf{HPOD} & \textbf{HyperEns} & 0.0607           & \textbf{HPOD} & ES                & 0.0016           \\
\textbf{HPOD} & GB                & 0.0017           & \textbf{HPOD} & Default           & 0.0029      \\
\bottomrule
\end{tabular}}
% \vspace{0.05in}
\end{table}

==> backup_aaai/tables/pairs.tex <==
\begin{table}[!ht]
    \footnotesize
    \label{table:all_pairs}
    \vspace{-0.1in}
    \begin{subtable}[t]{.48\textwidth}
        \centering
        \caption{On RAE, \method is statistically better than all baselines.}\label{table:rae_pairs}
        \vspace{-0.05in}
            \scalebox{0.82}{
           \begin{tabular}{lll|lll}
            \toprule
            \textbf{Ours} & \textbf{baseline} & \textbf{p-value} & \textbf{Ours} & \textbf{baseline} & \textbf{p-value} \\
            \midrule
            \textbf{HPOD} & AS                & 0.0309           & \textbf{HPOD} & ISAC              & 0.0028           \\
            \textbf{HPOD} & Random            & 0.0014           & \textbf{HPOD} & MetaOD            & 0.0398           \\
            \textbf{HPOD} & HyperEns          & 0.0382           & \textbf{HPOD} & MinLoss           & 0.0003           \\
            \textbf{HPOD} & GB                & 0.0002           & \textbf{HPOD} & HPOD\_0            & 0.0201    \\
            \bottomrule
            \end{tabular}}
    \end{subtable}
    \vspace{-0.05in}
    
    \begin{subtable}[t]{.48\textwidth}
        \centering
        \caption{On LOF, \method is statistically better than all (except HyperEnsemble (HE)), including the \textit{default} HP setting.}\label{table:lof_pairs}
                \vspace{-0.05in}
            \scalebox{0.82}{
           \begin{tabular}{lll|lll}
            \toprule
            \textbf{Ours} & \textbf{baseline} & \textbf{p-value} & \textbf{Ours} & \textbf{baseline} & \textbf{p-value} \\
            \midrule
            \textbf{HPOD} & AS                & 0.0023           & \textbf{HPOD} & ISAC              & 0.0246           \\
            \textbf{HPOD} & Random            & 0.0001           & \textbf{HPOD} & MetaOD            & 0.0088           \\
            \textbf{HPOD} & \textbf{HyperEns} & 0.0607           &   \textbf{HPOD} & Default           & 0.0029            \\
            \textbf{HPOD} & GB                & 0.0017           & \textbf{HPOD} & HPOD\_0                & 0.0016          \\
            \bottomrule
            \end{tabular}}
    \end{subtable}
    \vspace{-0.05in}

    \begin{subtable}[t]{.48\textwidth}
        \centering
        \caption{On iForest, \method is statistically better than all baselines, including the \textit{default} HP setting.}\label{table:iforest_pairs}
                \vspace{-0.05in}
            \scalebox{0.82}{
           \begin{tabular}{lll|lll}
            \toprule
            \textbf{Ours} & \textbf{baseline} & \textbf{p-value} & \textbf{Ours} & \textbf{baseline} & \textbf{p-value} \\
            \midrule
\textbf{HPOD} & AS                & 0.0055           & \textbf{HPOD} & ISAC              & 0.0088           \\
\textbf{HPOD} & Random            & 0.0003           & \textbf{HPOD} & MetaOD            & 0.0289           \\
\textbf{HPOD} & HyperEns & 0.0484           &        \textbf{HPOD} & Default           & 0.0013    \\
\textbf{HPOD} & GB                & 0.0027           & \textbf{HPOD} & HPOD\_0                & 0.003                \\
            \bottomrule
            \end{tabular}}
    \end{subtable}
    \vspace{-0.1in}
    \caption{Pairwise statistical test results between \method and baselines by Wilcoxon signed rank test. Statistically better method shown in \textbf{bold} (both marked \textbf{bold} if no significance).}
% \vspace{-0.05in}
\end{table}

==> tables/RAE_pairs.tex <==
\begin{table}[h]
% \scriptsize
\caption{
Pairwise statistical test results between \method and baselines by Wilcoxon signed rank test. Statistically better method shown in \textbf{bold} (both marked \textbf{bold} if no significance). For HPO on RAE, \method is statistically better than all. }\label{table:rae_pairs}
 \vspace{-0.1in}
\scalebox{0.87}{
\begin{tabular}{lll|lll}
\toprule
\textbf{Ours} & \textbf{baseline} & \textbf{p-value} & \textbf{Ours} & \textbf{baseline} & \textbf{p-value} \\
\midrule
\textbf{HPOD} & AS                & 0.0309           & \textbf{HPOD} & ISAC              & 0.0028           \\
\textbf{HPOD} & Random            & 0.0014           & \textbf{HPOD} & MetaOD            & 0.0398           \\
\textbf{HPOD} & HyperEns          & 0.0382           & \textbf{HPOD} & MinLoss           & 0.0003           \\
\textbf{HPOD} & GB                & 0.0002           & \textbf{HPOD} & HPOD\_0            & 0.0201    \\
\bottomrule
\end{tabular}}
% \vspace{0.05in}
\end{table}

==> tables/iforest_pairs.tex <==
\begin{table}[h]
% \scriptsize
\caption{
Pairwise statistical test results between \method and baselines by Wilcoxon signed rank test. Statistically better method shown in \textbf{bold} (both marked \textbf{bold} if no significance).
For HPO on iForest, \method is statistically better than all, including the \textit{default} HP setting.}\label{table:iforest_pairs}
 \vspace{-0.1in}
\scalebox{0.87}{
\begin{tabular}{lll|lll}
\toprule
\textbf{Ours} & \textbf{Baseline} & \textbf{p-value} & \textbf{Ours} & \textbf{Baseline} & \textbf{p-value} \\
\midrule
\textbf{HPOD} & AS                & 0.0055           & \textbf{HPOD} & ISAC              & 0.0088           \\
\textbf{HPOD} & Random            & 0.0003           & \textbf{HPOD} & MetaOD            & 0.0289           \\
\textbf{HPOD} & \textbf{HyperEns} & 0.0484           & \textbf{HPOD} & ES                & 0.003            \\
\textbf{HPOD} & GB                & 0.0027           & \textbf{HPOD} & Default           & 0.0013               \\
\bottomrule
\end{tabular}}
% \vspace{0.05in}
\end{table}

==> tables/lof_pairs.tex <==
\begin{table}[h]
% \scriptsize
\caption{
Pairwise statistical test results between \method and baselines by Wilcoxon signed rank test. Statistically better method shown in \textbf{bold} (both marked \textbf{bold} if no significance).
For HPO on LOF, \method is statistically better than all (except HyperEnsemble), including the \textit{default} HP setting.}\label{table:lof_pairs}
 \vspace{-0.1in}
\scalebox{0.87}{
\begin{tabular}{lll|lll}
\toprule
\textbf{Ours} & \textbf{Baseline} & \textbf{p-value} & \textbf{Ours} & \textbf{Baseline} & \textbf{p-value} \\
\midrule
\textbf{HPOD} & AS                & 0.0023           & \textbf{HPOD} & ISAC              & 0.0246           \\
\textbf{HPOD} & Random            & 0.0001           & \textbf{HPOD} & MetaOD            & 0.0088           \\
\textbf{HPOD} & \textbf{HyperEns} & 0.0607           & \textbf{HPOD} & ES                & 0.0016           \\
\textbf{HPOD} & GB                & 0.0017           & \textbf{HPOD} & Default           & 0.0029      \\
\bottomrule
\end{tabular}}
% \vspace{0.05in}
\end{table}
